Passivity-preserving splitting methods for rigid body systems

A rigid body model for the dynamics of a marine vessel, used in simulations of offshore pipe-lay operations, gives rise to a set of ordinary differential equations with controls. The system is input-output passive. We propose passivity-preserving splitting methods for the numerical solution of a class of problems which includes this system as a special case. We prove the passivity-preservation property for the splitting methods, and we investigate stability and energy behaviour in numerical experiments. Implementation is discussed in detail for a special case where the splitting gives rise to the subsequent integration of two completely integrable flows. The equations for the attitude are reformulated on $SO(3)$ using rotation matrices rather than local parametrizations with Euler angles.

==> Submission arXiv/Chapters/1_Introduction.tex <==
\section{Introduction}


In this paper we propose passivity preserving splitting methods for the control of input-output passive rigid body systems, and in particular for a model of a marine vessel. The preservation of passivity under numerical discretization is not well known  in the literature. We here propose a simple and general technique to achieve passivity-preservation under numerical discretization when using splitting methods. This technique is applicable to a large class of input-output passive systems, of which the vessel model is a special example.

%In this paper we apply the methods to a system of ordinary differential equations  (ODEs) with controls arising as a model of a marine vessel. 
The control of vessel rigid body equations is important in the simulation of a number of offshore marine operations \cite{marinecontrolsystems}. One example is the simulation of pipeline installations sketched in Figure~\ref{fig2}. %where an interaction of a vessel and a thin flexible pipe attached to it is demonstrated. 
%This marine operation requires the use of accurate models solved with reliable numerical methods.
\begin{figure}
\centering
\includegraphics[width=11cm]{Figures/pipe-lay}
\caption{The offshore pipe-lay process. The purpose build pipeline vessel uses heavy tension equipment to clamp the pipe on to it. The pipe is then extended in a production line. The two main pipelay methods are the dominant S-lay (shown) and J-lay. In the S-lay method, the pipe is extended horizontally. The name S-lay comes from the S-shape of the pipe from vessel to seabed. A submerged supporting structure, called a stinger, controls curvature and ovalization in the upper part (overbend). Pipe tension controls the curvature in the lower curve (sagbend). The strain must be checked to stay within limits for buckling and ovalization. See \cite{jensen09mac} and the references therein for more details.\label{fig2}}%In deep waters, the increased pipe weight, and consequent tension, makes it difficult to maintain a stinger supported overbend. The J-lay method is therefore preferred. Here the pipe is extended near vertically, forming a J-shaped curve. This eliminates the overbend. See \cite{jensen09mac} and the references therein for more details.}
\end{figure}
The pipe-laying process comprises the modeling of two interacting structures, a vessel and a pipe. It is usual to model the vessel as a torqued rigid body with control, and the long and thin pipe as a rod. %Environmental forces such as sea and wind effects must in general be accounted for in the model. For this problem t
The parameters to control are the vessel position and velocity, the pay-out speed, and the pipe tension. The control objectives are to determine the position of the touchdown point of the pipe, and to avoid critical deformations and structural failures  \cite{jensen09mac}, \cite{jensen10anp}. The design of damping forces and controls must ensure that the resulting system is input-output passive, i.e. an energy conservation/dissipation property must be satisfied.  

The full pipe-lay problem has already been simulated in \cite{jensen10anp}, using local parametrisations based on Euler angles for both the pipe and the vessel model and with standard numerical techniques. The focus in this paper is %on developing efficient and robust solvers for 
the the passivity preserving integration of the vessel rigid-body model. %, since this is the only part of the vessel-rod multibody system which can be controlled, and also since the boundary conditions of the rod come from the vessel rigid body equations. 
%The numerical approach we here pursue is aimed at respecting the properties of passivity of the control system, and to respect the manifold structure of the equations, the attitude rotation evolves on the Lie group $SO(3)$.

We consider the six degrees of freedom model for the dynamics of a
marine vessel given in  \cite{jensen10anp} (see also \cite{marinecontrolsystems} and \cite{perez07kmf}), which expressed in matrix-vector form
is
\begin{align}
\dot{\mbox{\boldmath $\eta$}}&=J(\mbox{\boldmath $\eta$})\mbox{\boldmath $\nu$}, \nonumber \\
M\dot{\mbox{\boldmath $\nu$}} + C(\mbox{\boldmath $\nu$})\mbox{\boldmath $\nu$}
 + D(\mbox{\boldmath $\nu$})\mbox{\boldmath $\nu$} + \mathbf{g}(\mbox{\boldmath $\eta$}) &=
\mbox{\boldmath $\tau$} +\mathbf{\mathcal{X}}+ \mathbf{w}, \label{eq:vesseleq}
\end{align}

\noindent where $\mbox{\boldmath $\eta$}$ and $\mbox{\boldmath $\nu$}$ are  generalised position and velocity respectively, $M$ is the system inertia matrix, $C(\mbox{\boldmath $\nu$})$ the skew-symmetric Coriolis-centripetal matrix, $D(\mbox{\boldmath $\nu$})$ the symmetric damping matrix, $\mathbf{g}(\mbox{\boldmath $\eta$})$ the vector of gravitational and buoyancy forces and moments, $\mbox{\boldmath $\tau$}$ the vector of control inputs, $\mathbf{\mathcal{X}}$ the forces and moments from the pipe, and $\mathbf{w}$ environmental disturbances such as wind, waves and currents,  see section~\ref{model} and \ref{controls} for details.  The position variables $\mbox{\boldmath $\eta$}$ include the three Euler angles representing the attitude of the body and evolving on the Lie group $SO(3)$. We reformulate the equations using rotation matrices, and provide numerical approximations that preserve the structure of this manifold.

%We consider a general setting for input-output passive systems in which controlled rigid body systems as the
This vessel model \eqref{eq:vesseleq} is a special example of an input-output passive systems, and in particular an input-state-output port-Hamiltonian system, \cite{VanderSchaft06pHs}. The passivity of the vessel system follows directly from the passivity of port-Hamiltonian systems (see Section~\ref{passivity}).
%The vessel  ODE system is input-output passive as can be easily shown by writing the vector field of the system using a skew-symmetric matrix which multiplies the gradient of a Hamiltonian function, to which are added dissipative forces and controls (see section~\ref{passivity}). 
Our proposed numerical integration methods are splitting methods, a class of integration methods very well known in the geometric numerical integration literature \cite{gni06hairer}. % because of their structure preserving properties, but less popular in the multi-body dynamics community. 
We propose to split systems of the type \eqref{eq:vesseleq} into a conservative part, and a part comprising torque, dissipative forces and controls. 
We prove passivity of the proposed splitting methods for the general class of input-state-output port-Hamiltonian systems.
%preserve the passivity of the system under discretization by splitting  the skew-symmetric matrix in the sum of two skew-symmetric terms. %We propose an efficient splitting-and-composition technique, obtaining methods of order $2$.
%We formulate the torqued/controlled rigid body equations using Euler parameters and rotation matrices.%, $4$ and $6$. 
%To measure the performance of the numerical techniques we are not only looking at the behaviour of the global error but also in terms of preservation of the total energy of the system. We shall also remark on the passivity of this system under the given assumptions. It has been shown in \cite{jensen10anp} that the rigid body vessel equations are input-output passive (with input \mbox{\boldmath $\tau$} and output \mbox{\boldmath $\nu$})
%Since the system is input-output passive, we consider splittings of the system that preserve passivity under discretization. It turns out that for the vessel 
%equations this can be achieved 
%The two resulting parts are a conservative, free rigid body part, and a part comprising torque, dissipative forces and controls.  %So the equations can be easily integrated numerically by a splitting and composition technique. %where the vessel equations are split into a free rigid body part and a damping and control part.
%The free rigid body equations comprise the kinematics of rotations and are completely integrable, an explicit solution can be obtained and computed numerically to high accuracy by using Jacobi elliptic functions \cite{celledoni06ets}, \cite{celledoni08tec}, \cite{celledoni10frb}. %


%The free rigid body equations are completely integrable, and an explicit solution can be obtained and computed numerically to high accuracy by using Jacobi elliptic functions \cite{celledoni06ets}, \cite{celledoni08tec}, \cite{celledoni10frb}.
%can be solved with a method proposed in \cite{celledoni06ets}, \cite{celledoni08tuo} where the angular momentum is accurately and efficiently computed by using Jacobi elliptic functions, and the attitude rotation is either computed exactly or obtained using a Lie group method based on the Magnus expansion.
For a simplified model, where  %the contribute of the linear momentum to the kinetic energy is
both control and damping are linear with constant coefficients and the mass matrix has a special structure, the two individual flows are completely integrable, and we discuss the implementation details of their exact solution.
%the remaining part of the equations can be easily solved exactly by the variation of constants formula. For the case when the remaining part of the system is a nonlinear vector field (due to quadratic damping terms and when allowing for completely general added mass) one can solve this part of the splitting by an energy-preserving/energy-dissipative integrator \cite{mclachlanDG} and still ensure passivity of the discrete system. %an exponential integrator is proposed for this part of the equations, see appendix.


In the presence of PID (proportional-integral-derivative) controls, $\mbox{\boldmath $\tau$}$ depends on $\mbox{\boldmath $\nu$} $, on $\mbox{\boldmath $\eta$}$ and on the integral of $\mbox{\boldmath $\eta$}$ over time. 
We include this integral as an extra unknown to the system to avoid explicit time dependence in the system of equations. %We adopt optimised splitting techniques devised by Blanes et al. \cite{blanes}, to obtain high order. The result is an efficient method.
%We also give a proof of passivity of the resulting system of equations.

%The splitting methods must be appropriately adapted to this situation. We approach this in the simplest possible way by treating time as a new variable, and adding this new variable to the system.

Finally, we make a numerical study of the order and 
% stability behaviour of the splitting methods depending on the step-size. T
the energy behaviour of the methods. The results are compared with those given by explicit Runge-Kutta methods. %The splitting methods here proposed are robust, and show improved energy and global error behaviour compared to explicit Runge-Kutta methods of the same order. %, especially for long time simulations (with small damping) and large step-sizes.
% fully discrete model, regarding the preservation of total energy of the system. %input-output passivity property of the original system.

The outline of the paper is as follows: 
in Section 2 we remark on the passivity of this system, describe the details of the splitting and composition techniques and show their input-output passivity; in Section 3 we describe the vessel equations and describe the implementation details; in Section 4 we report our numerical results illustrating the performance of the methods; Section 5 is devoted to conclusions.







==> Submission arXiv/Chapters/2_Vessel_model.tex <==
\def\Z3x3{0{\ensuremath{_{3\times3}}}}
\def\I3x3{I{\ensuremath{_{3\times3}}}}

\section{A vessel rigid body model}
\label{model}

We give now more details about the system \eqref{eq:vesseleq} presented in the introduction. We will eventually show that it can be cast in the format of the system \eqref{eq:xiDiff}.
The generalized velocity vector $\mbox{\boldmath $\nu$}=
[\mathbf{v}^T, \mbox{\boldmath $\omega$}^T]^T \in \mathbf{R}^6$ lies in the body frame, where $\mathbf{v},\mbox{\boldmath $\omega$ } \in \mathbf{R}^3$ denote respectively the linear velocity and the angular velocity. The generalized position vector $\mbox{\boldmath $\eta$} = [\mathbf{x}^T, 
\mbox{\boldmath $\theta$}^T]^T \in \mathbf{R}^6$ lies in the spatial frame. Here $\mathbf{x}\in\mathbf{R}^3$ is the position vector and the components of $\mbox{\boldmath $\theta$}=[\phi,\theta,\psi]^T$ are the Euler angles, which provide a local representation of the attitude of the vessel. The attitude of the body evolves on the Lie group $SO(3)$, which is a manifold. The elements of $SO(3)$ can be represented as $3\times 3$ rotation matrices. If $Q$ is sufficiently close to the identity, then  the conversion between Euler angles and rotation matrices is %the two choices of coordinates is
\begin{equation}
\label{EulerangtoRot}
Q=\Psi(\mbox{\boldmath $\theta$})=R_{z,\psi }\,R_{y,\theta}\,R_{x,\phi},\quad \mbox{\boldmath $\theta$}=[\phi,\theta,\psi]^T,
\end{equation}
with
{\small
$$R_{x,\phi}=\left[
\begin{array}{ccc}
1 & 0 & 0 \\
0 & \cos(\phi) &-\sin(\phi)\\
0 & \sin(\phi) & \cos(\phi)
\end{array}
\right],\, R_{y,\theta}=\left[ \begin{array}{ccc}
\cos(\theta) & 0 & \sin(\theta) \\
0 & 1 &0\\
 -\sin(\theta) & 0 & \cos(\theta)
\end{array}
\right],\, 
R_{z,\psi}=\left[ \begin{array}{ccc}
\cos(\psi) & -\sin(\psi) & 0 \\
 \sin(\psi) & \cos(\psi) & 0\\
0 & 0 &1
\end{array}
\right], $$
}and $\Psi$ is a local diffeomorphism, i.e. $\Psi$ is invertible for $Q$ close to the identity.
Notice that $Q$ can always be transported close to the identity by multiplying with a rotation $Q_0^{-1}\approx Q^{-1}$ so that $Q_0^{-1}Q=\Psi(\mbox{\boldmath $\theta$})$.
The kinematic equation associated with \eqref{eq:vesseleq} is
\begin{equation}
\label{eq:kinematics}
\dot{\mbox{\boldmath $\eta$}} = J(\mbox{\boldmath $\eta$})
\mbox{\boldmath $\nu$},\qquad J(\mbox{\boldmath $\eta$}) = \left[\begin{array}{cc} Q & \Z3x3 \\
\Z3x3 & \Pi_e^{-1}Q \end{array} \right],
\end{equation}

\noindent with

$$
\Pi_e = \left[\begin{array}{ccc} \cos(\theta)\cos(\psi) & -\sin(\psi) & 0 \\
\cos(\theta)\sin(\psi) & \cos(\psi) & 0 \\
-\sin(\theta) & 0 & 1 \end{array} \right],
$$
see also \cite{marinecontrolsystems}, \cite{safstrom09mas}. 
We then get the kinematic equation $\dot{\mbox{\boldmath $\theta$}}=\Pi_e^{-1}Q\,\mbox{\boldmath $\omega$}$ for the Euler angles, which can be obtained by differentiating \eqref{EulerangtoRot} and is also valid locally. The matrix $\Pi_e$ is not invertible for $\theta=\pm \frac{\pi}{2}$ and $\psi=\pm \frac{\pi}{2}$. To avoid these singularities, we rewrite this kinematic equation 
as an equation for $Q$ 
\begin{equation}
\label{eq:attitudeSO3}
\dot{Q}=Q\,\widehat{\mbox{\boldmath $\omega$}}.
\end{equation}
This equation is globally defined on $SO(3)$.
%
The rotation matrix $Q$ transforms vectors in the body fixed frame $\{b\}$  
to vectors in the spatial frame $\{s\}$ \footnote{$Q:=R_b^e$ in the notation of \cite{perez07kmf} and \cite{marinecontrolsystems}.}.
Here
$$\widehat{\mbox{\boldmath $\,\,$}}:\mathbb{R}^3 \rightarrow \mathfrak{so}(3),\qquad \widehat{\mbox{\boldmath $\omega$}}=\left[
\begin{array}{ccc}
0 & -\omega_3 & \omega_2 \\
\omega_3 & 0 &-\omega_1\\
-\omega_2 & \omega_1 & 0
\end{array}
\right],$$
is the hat-map, and  $\mathfrak{so}(3)$ is the Lie algebra of $SO(3)$, consisting of $3\times 3$ skew-symmetric matrices, for further details see \cite{muller}.



%


Following \cite{lamb} (p. 151) and \cite{Kirchhoff}, equations \eqref{eq:vesseleq} can be obtained defining  the kinetic energy of the system to be
$$K=\frac{1}{2}\mbox{\boldmath $\nu$}^TM\mbox{\boldmath $\nu$},$$ leading to Kirchhoff's equations
\begin{eqnarray}
\label{kirchoff1}
\frac{d}{dt}\frac{\partial K}{\partial \mathbf{v}}& = & \frac{\partial K}{\partial \mathbf{v}} \times \mbox{\boldmath $\omega$}+ F_v,\\
\label{kirchoff2}
\frac{d}{dt}\frac{\partial K}{\partial \mbox{\boldmath $\omega$}}& = & \frac{\partial K}{\partial \mbox{\boldmath $\omega$}} \times \mbox{\boldmath $\omega$}+\frac{\partial K}{\partial\mathbf{v}}\times \mathbf{v}+ F_{\omega},
\end{eqnarray}
where $[\mathbf{p}^T, \mathbf{m}^T]^T:=\frac{\partial K}{\partial \mbox{\boldmath $\nu$}}=M\mbox{\boldmath $\nu$}$, and with $F_v$ and $F_{\omega}$ the external force and torque respectively. These include the damping forces, the gravitational and buoyancy forces, the control inputs, the forces due to the pipe, and environmental forces.%
In absence of external forces, the obtained equations have a Lie-Poisson structure, and can be derived by variational methods \cite{holm} (p.129). We refer to \cite{marsden99IMS} (p. 421) for the general description of the Euler-Poincare reduction on Lie groups (the relevant Lie group in this case is $SE(3)$). For formulations obtained applying the Hamilton-Pontriagin principle, see  \cite{BM}, and for the inclusion of external forces see \cite{marsdenwest} (p. 421).

If we set
\begin{equation}
\label{RBmomenta}
\mathbf{p}:=\frac{\partial K}{\partial \mathbf{v}},\qquad   \mathbf{m}:= \frac{\partial K}{\partial \mbox{\boldmath $\omega$}}, \quad 
\left[  \begin{array}{c}
\mathbf{p}\\
 \mathbf{m}
\end{array}
\right]= M \, \mbox{\boldmath $\nu$},
\end{equation}
the general form of the skew-symmetric Coriolis-centripetal matrix is
\begin{equation}
\label{Coriolisgeneral}
C(\mbox{\boldmath $\nu$}) = -\left[
\begin{array}{cc}
\Z3x3 & \widehat{\frac{\partial K}{\partial \mathbf{v}}}\\[0.1cm]
\widehat{\frac{\partial K}{\partial \mathbf{v}}} & \widehat{\frac{\partial K}{\partial \mbox{\boldmath $\omega$}}}
\end{array}
\right]=-\left[
\begin{array}{cc} 
\Z3x3 & \hat{\mathbf{p}} \\ 
 \hat{\mathbf{p}} & \hat{\mathbf{m}} \end{array} \right].
\end{equation}


Since $K$ is a homogeneous quadratic polynomial in  the components of $\mbox{\boldmath $\nu$}$, only the symmetric part of $M$ plays a role, and we can assume $M$ to be symmetric. The matrix $M$ can be split into a rigid body part $M_{RB}$ and a part for
added mass $M_A$. The same can be done for the kinetic energy $K=K_{RB}+K_{A}$ and the Coriolis-centripetal matrix $C(\mbox{\boldmath $\nu$})=C_{RB}(\mbox{\boldmath $\nu$})+C_A(\mbox{\boldmath $\nu$})$. 
Letting the origin of the body fixed frame coincide with the center of gravity in our model, the rigid body system inertia matrix $M_{RB}$ has the simple form
\begin{equation}
\label{MRB}
M_{RB} = \left[\begin{array}{cc} m_v\I3x3 & \Z3x3 \\
\Z3x3 & T \end{array} \right],
\end{equation}
where $m_v$ is the mass of the vessel, $\I3x3$ is the 3-dimensional identity
matrix, and $T$ is the inertia tensor.
The added mass term $M_A$ is a symmetric matrix, and 
%when the origin is in the center of gravity, $M_A$ can also be approximated by a  diagonal matrix (see \cite{marinecontrolsystems} p. 98 ).
we notice that when $M_A$ is set to zero, due to the structure of $M_{RB}$, the term $\frac{\partial K}{\partial\mathbf{v}}\times \mathbf{v}$ in \eqref{kirchoff2} vanishes. 

With this simplification, we get 
$$
\frac{\partial K}{\partial \mathbf{v}}=m_v  \mathbf{v},\qquad    \frac{\partial K}{\partial \mbox{\boldmath $\omega$}}=T \mbox{\boldmath $\omega$},
$$
and from \eqref{kirchoff1} and \eqref{kirchoff2} we deduce that  the rigid body Coriolis-centripetal matrix in this case can be rewritten in the form
%$C_{RB}(\mbox{\boldmath $\nu$})$ from \cite{marinecontrolsystems} is

$$
C_{RB}(\mbox{\boldmath $\nu$}) = \left[\begin{array}{cc} m_v\hat{\mbox{\boldmath $\omega$}}
& \Z3x3 \\ \Z3x3 & -\widehat{T\mbox{\boldmath $\omega$}} \end{array} \right].
$$
In the general case, 
%if we set
%$$
%\mathbf{p}:=\frac{\partial K}{\partial \mathbf{v}},\qquad   \mathbf{m}:= \frac{\partial K}{\partial \mbox{\boldmath $\omega$}},
%$$
%we have
%$$
%C(\mbox{\boldmath $\nu$}) = -\left[\begin{array}{cc} \Z3x3 & \hat{\mathbf{p}}}
 %\\ \hat{\mathbf{p}}} & \hat{\mathbf{m}} \end{array} \right].
%$$
$M$ is symmetric and %constant, it can be diagonalised via a constant orthogonal transformation, and, after an appropriate change of variables, $M$ can be assumed to be diagonal, 
$C(\mbox{\boldmath $\nu$})$ is  given by \eqref{Coriolisgeneral}, with $\mathbf{p}$ and $\mathbf{m}$  given by \eqref{RBmomenta}. We will here make the additional assumption that $M$ is block diagonal, (see \cite{marinecontrolsystems} p. 98 about this assumption), and that it is diagonal when the origin of the body frame is in the center of gravity. %where $m_v$ is now an appropriate  $3\times 3$ diagonal matrix. 

%Even though this is not so in general, we will hereafter assume $M_A=0$. Such simplification does not compromise the generality of the method proposed in this paper\footnote{In the general case $M_A$ is non zero and is not diagonal, however often because of symmetry considerations for the vessel, the matrix $M$ is symmetric and is close to being block diagonal, this fact can be exploited to generalise the method we propose in next section.}.




We have so far accounted for the first two terms in the equations  \eqref{eq:vesseleq}, and we will in the sequel describe the remaining forces and moments.

The term $\mathbf{g}(\mbox{\boldmath $\eta$})$ from Equation (\ref{eq:vesseleq}) takes restoring
forces and moments into account. In the model adopted in \cite{jensen09mac},
$\mathbf{g}(\mbox{\boldmath $\eta$})$, which lies in the body frame, is given as

$$
\mathbf{g}(\mbox{\boldmath $\eta$}) = \left[\begin{array}{c} Q^T \mathbf{g}_t^s \\ Q^T \mathbf{g}_r^s \end{array}
\right],
$$

\noindent where the superscript $s$ denotes that the vector lies in the spatial frame. 

Again following \cite{jensen09mac}, we have for the rotational part

$$
\mathbf{g}_r^s = (Q\mathbf{r}_r^b)\times(m_vg\mathbf{e}_3),
$$

\noindent where $g$ is the gravitational acceleration and $\mathbf{r}_r^b$ is the moment arm
in the body frame. The latter can be expressed as %- after the removal of the Euler angle
%dependence -


$$
\mathbf{r}_r^b = \left[\begin{array}{c} \overline{GM}_L (Q\mathbf{e}_1)^T\mathbf{e}_3 \\
\overline{GM}_T (Q\mathbf{e}_2)^T\mathbf{e}_3 \\ 0 \end{array}\right],
$$

\noindent where $\overline{GM}_L$ and $\overline{GM}_T$ are the longitudinal and the
transverse metacentric heights of the vessel, respectively.

The vector $\mathbf{g}_t^s$ accounts for buoyancy forces, and can be modelled as
$$
\mathbf{g}_t^s = g \rho_w A_{wp}(z-z_{eq}) \mathbf{e}_3,
$$
following an approach similar to that in \cite{jensen10anp}. Here $\rho_w$ is the density of water, $A_{wp}$ is the water plane area and $z_{eq}$ is the equilibrium water level. These forces can be directly included by adding a potential energy term to the kinetic energy $K=\frac{1}{2}\mbox{\boldmath $\nu$}^TM\mbox{\boldmath $\nu$}$, when considering the Lie group models of \cite{holm}, \cite{marsden99IMS} and \cite{BM}.


For the positive definite damping matrix $D(\mbox{\boldmath $\nu$})$, we also make use of a common simplifying assumption that the matrix is diagonal when the origin of the fixed body coordinate system coincides with the center of gravity. %????In addition, %due to the slow-speed assumption, 
%we will neglect to begin with the nonlinear damping terms, considering the case of nonlinear quadratic damping in the appendix.
 %i.e. that the damping matrix is constant  \cite{marinecontrolsystems}. 
 We therefore represent this matrix as
$$
D(\mbox{\boldmath $\nu$}) = \left[\begin{array}{cc} D_t(\mathbf{v})
& \Z3x3 \\ \Z3x3 & D_r (\mbox{\boldmath $\omega$}) \end{array} \right],
$$
where $D_t,D_r \in  \mathbb{R}^{3\times 3}$ are positive definite diagonal matrices.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Right hand side forces}\label{controls}

Let us now consider  the term $\mbox{\boldmath $\tau$} $ in \eqref{eq:vesseleq}.
Following the model presented in \cite{jensen10anp} we set

\begin{equation}
\begin{array}{rcl}
%\label{tau1}
\mbox{\boldmath $\tau$} &=& -J^T(\mbox{\boldmath $\eta$}) \mbox{\boldmath $\tau$}_{PID}, \\
%\label{tau2}
\mbox{\boldmath $\tau$}_{PID} &=& K_p \tilde{\mbox{\boldmath $\eta$}} + K_d \dot{\tilde{\mbox{\boldmath $\eta$}}}
+ K_i\int_{t_0}^{t}\! \tilde{\mbox{\boldmath $\eta$}}(\sigma) \,d\sigma,
\label{eq:control_tau}
\end{array}
\end{equation}

\noindent where the matrices

\begin{equation}
K_p=\left[\begin{array}{cc}K_p^{t} & \Z3x3 \\ \Z3x3 & K_p^{r}\end{array}\right], \hspace{4mm}
K_d=\left[\begin{array}{cc}K_d^{t} & \Z3x3 \\ \Z3x3 & K_d^{r}\end{array}\right],  \hspace{2mm} \text{and} \hspace{2mm}
K_i=\left[\begin{array}{cc}K_i^{t} & \Z3x3 \\ \Z3x3 & K_i^{r}\end{array}\right],
\label{eq:control_gains}
\end{equation}

\noindent are called controller gains, and
$\tilde{\mbox{\boldmath $\eta$}} := \mbox{\boldmath $\eta$} - \mbox{\boldmath $\eta$}_{ref}$.
%and
%
%$$
%J(\mbox{\boldmath $\eta$}) = \left[\begin{array}{cc} Q & 0 \\
%0 & \Pi_e^{-1}Q \end{array} \right],
%$$
%
%\noindent with
%
%$$
%\Pi_e = \left[\begin{array}{ccc} \cos(\theta)\cos(\psi) & -\sin(\psi) & 0 \\
%\cos(\theta)\sin(\psi) & \cos(\psi) & 0 \\
%-\sin(\theta) & 0 & 1 \end{array} \right],
%$$
%
%\noindent which depends on the Euler angles - n

This formulation of the control forces is based on the use of Euler angles, $\mbox{\boldmath $\theta$}$, to locally parametrize the rotation matrix $Q$.
%This formulation of the control forces is based on the use of Euler angles $\mbox{\boldmath $\theta$}$ for the local parametrization of the rotation $Q$, \eqref{EulerangtoRot}. 
Away from singularities, i.e. for $Q$ close to the identity, we have $\mbox{\boldmath $\theta$}=\Psi^{-1}( Q)$, with $\Psi$ given by \eqref{EulerangtoRot}.  A reformulation of the control forces using only $Q$ and the angular velocity $\omega$ will require a different design of the controller gains \eqref{eq:control_gains} and will not be pursued here.

In the case where $K_i$ is different from the zero matrix, we introduce a new set of unknowns
$$
\mbox{\boldmath $\varphi$}:=\int_{t_0}^t \tilde{\boldsymbol{\eta}} (\sigma)\, d\sigma,
$$
and add a corresponding new set of equations to the system \eqref{eq:vesseleq}
$$\dot{\mbox{\boldmath $\varphi$}}= \tilde{\boldsymbol{\eta}}(t),\qquad {\mbox{\boldmath $\varphi$}}(t_0)=0.$$
The integral term in $\mbox{\boldmath $\tau$}_{PID}$ can then be written as
$$\int_{t_0}^{t}\! \tilde{\boldsymbol{\eta}}(\sigma) \,d\sigma={\mbox{\boldmath $\varphi$}}, \qquad {\mbox{\boldmath $\varphi$}}=({\mbox{\boldmath $\varphi$}}_{\mathbf{x}}, {\mbox{\boldmath $\varphi$}}_{\boldsymbol{\theta}}),$$
(as with ${\boldsymbol{\theta}}$, the equation for ${\mbox{\boldmath $\varphi$}}_{\boldsymbol{\theta}}$ is valid locally). %     
Note that the system of equations is then autonomous, i.e. does not explicitly depend on $t$.
Though not required, we let $\mathbf{w} = \mathbf{0}$ for simplicity in what follows. 
In \cite{jensen10anp} the pipe is assumed to be fixed to the center of gravity of the vessel. The forces and moments from the pipe on the vessel, $\mathbf{\mathcal{X}}$, depend on the stress resultant and stress couple of the pipe.  Since the modeling and simulation of the pipe structure is not the focus of this paper, these forces are not taken into account. 
 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The set of equations}

Using the explicit expressions for the right hand side forces, the system \eqref{eq:vesseleq} can be written as 

\begin{align}
\dot{\mathbf{p}} &= \mathbf{p}\times \mbox{\boldmath $\omega$} -\left(D_t(\mathbf{v})\mathbf{v}+Q^T\mathbf{g}_t^s(\mathbf{x})-\mbox{\boldmath $\tau$}_t\right), \nonumber  \\ 
\dot{\mathbf{m}} &= \mathbf{m} \times \mbox{\boldmath $\omega$}+\mathbf{p}\times \mathbf{v} - \left(D_r(\mbox{\boldmath $\omega$})\mbox{\boldmath $\omega$}+Q^T\mathbf{g}_r^s(Q)-\mbox{\boldmath $\tau$}_r\right), \label{eq:vessel}\\
\dot{Q}&=Q\,\widehat{\mbox{\boldmath $\omega$}}, \nonumber \\
\dot{\mathbf{x}} &= Q\,\mathbf{v}, \nonumber
\end{align}
with
\begin{align}
\mbox{\boldmath $\tau$}_r  &= -\left(\Pi_e^{-1}Q\right)^T(K_p^{r}\tilde{\mbox{\boldmath $\theta$}}
+ K_d^{r}\dot{\tilde{\mbox{\boldmath $\theta$}}} + K_i^{r} \mbox{\boldmath $\varphi$}_{\boldsymbol{\theta}} ), \label{controls1} \\
\boldsymbol{\tau}_t &= -Q^T \left(K_p^{t}\tilde{\mathbf{x}}
+ K_d^{t}\dot{\tilde{\mathbf{x}}} + K_i^{t} \mbox{\boldmath $\varphi$}_{\mathbf{x}}\right), \label{controls2} \\
\tilde{\mbox{\boldmath $\theta$}} &= \Psi^{-1}(Q)- \mbox{\boldmath $\theta$}_{ref}, 
\hspace{6mm}
\dot{\tilde{\mbox{\boldmath $\theta$}}} = \dot{\mbox{\boldmath $\theta$}} = \Pi_e^{-1}Q\, \mbox{\boldmath $\omega$} ,
\hspace{6mm}
\tilde{\mathbf{x}} = \mathbf{x}-\mathbf{x}_{ref}, \label{controls3}
\end{align}
and
\begin{align}
\dot{\mbox{\boldmath $\varphi$}}_{\boldsymbol{\theta}}&=\tilde{\mbox{\boldmath $\theta$}}, \nonumber\\
\dot{\mbox{\boldmath $\varphi$}}_{\mathbf{x}} &=\tilde{\mathbf{x}}. \nonumber
\end{align}


An alternative version of these equations, which uses Euler parameters to represent the attitude, is given in Appendix \ref{quatEq}.

\subsection{Passivity and splitting of the vessel equations}
For the vessel model, we now define $\mbox{\boldmath $\xi$} := [
\mathbf{p}^T, \mathbf{m}^T, \mathbf{q}_1^T, \mathbf{q}_2^T, \mathbf{q}_3^T, \mbox{\boldmath $\mu$}^T, \mathbf{x}^T ]$
with
$$
\mathbf{p} := m_v \mathbf{v}, \quad\mathbf{m} := T\boldsymbol{\omega},  \quad \mathbf{q}_i := Q^T\mathbf{e_i},\quad \mbox{\boldmath $\mu$}:=\mathcal{G}\mathbf{q}_3,
$$
with $m_v$ and $T$ diagonal and invertible matrices.
We take $H = H(\mbox{\boldmath $\xi$})$ to be the Hamiltonian of the system, given as the sum of the kinetic energy $K$ and the potential energy $U$. 
Defining
{\small
$$\mathcal{A}  := \mathrm{diag}(0,0,c), \quad \mathcal{G}  := m_v g\, \mathrm{diag}(\overline{GM}_L,\overline{GM}_T,0),\quad \tilde{\mathcal{G} } := \frac{1}{m_v g}\, \mathrm{diag}((\overline{GM}_L)^{-1},(\overline{GM}_T)^{-1},0),$$
}
and $c := g \rho_w A_{wp},$
we have
\begin{equation}
\label{Hamiltonian}
\begin{array}{lcl}K =\frac{1}{2}\mathbf{m}^T\ T^{-1} \mathbf{m} + \frac{1}{2}\mathbf{p}^T m_v^{-1}\mathbf{p},\\
U= \frac{1}{2}\mbox{\boldmath $\mu$}^T\tilde{\mathcal{G}}\mbox{\boldmath $\mu$}+\frac{1}{2}\mathbf{q}_1^T\mathbf{q}_1+\frac{1}{2}\mathbf{q}_2^T\mathbf{q}_2 + \frac{1}{2}\mathbf{q}_3^T\mathbf{q}_3+ \frac{1}{2}\mathbf{x}^T\mathcal{A}\mathbf{x},\\
H=K+U.
\end{array}
\end{equation}
Notice that the following identities hold
\begin{equation}
\label{gtsgrs}
\mathbf{g}_t^s=\mathcal{A}\, \mathbf{x},\quad Q^T\mathbf{g}_r^s=\mbox{\boldmath $\mu$}\times \mathbf{q}_3.
\end{equation}
We will in the next proposition replace the matrix equation $\dot{Q}=Q\hat{\boldsymbol{\omega}}$ in \eqref{eq:vessel} with three vector equations, one for each column $\mathbf{q}_i$, $i=1,2,3$, of $Q^T$.

\begin{Proposition}
\label{portHamSys}
The system \eqref{eq:vessel} can be written in the form
\begin{equation}
\label{eq:xiDiff1}
\dot{\mbox{\boldmath $\xi$}} = S(\mbox{\boldmath $\xi$})\nabla H(\mbox{\boldmath $\xi$}) -\tilde{I}\left(D(\mbox{\boldmath $\xi$})\mbox{\boldmath $\nu$} - \tilde{\mbox{\boldmath $\tau$}}\right),
\end{equation}
with
{\small
\begin{equation}
\label{eq:skewMat}
S(\mbox{\boldmath $\xi$}) := \begin{bmatrix} 
0_{3 \times 3} & \widehat{\mathbf{p}} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  0_{3 \times 3} &-Q^T \\ 
 \widehat{\mathbf{p}} &\widehat{\mathbf{m}} & 0_{3 \times 3} &0_{3 \times 3} & -\widehat{\mbox{\boldmath $\mu$}} & 0_{3 \times 3}  & 0_{3 \times 3}\\ 
 0_{3 \times 3} &  0_{3 \times 3} & -\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3} & 0_{3 \times 3} &0_{3 \times 3} & 0_{3 \times 3}\\
 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  -\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3}  &   0_{3 \times 3} & 0_{3 \times 3}\\
 0_{3 \times 3} & -\widehat{\mbox{\boldmath $\mu$}} &  0_{3 \times 3} &   0_{3 \times 3} &   -\widehat{T^{-1}\mathbf{m}} &   -\widehat{T^{-1}\mathbf{m}}\,\mathcal{G}  & 0_{3 \times 3}\\
 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & -\mathcal{G}\,\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3} & 0_{3 \times 3}\\
Q & 0_{3 \times 3} &  0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} & 0_{3 \times 3}
\end{bmatrix}, \ \ 
\tilde{I} := \begin{bmatrix} 
I{\ensuremath{_{6\times6}}} \\
0{\ensuremath{_{15\times6}}}
\end{bmatrix},
\end{equation}
}
$$D(\mbox{\boldmath $\xi$}):=D+\left[\begin{array}{cc} Q  & \Z3x3 \\
\Z3x3 & \Pi_e^{-1}Q \end{array} \right]^TK_d \left[\begin{array}{cc} Q & \Z3x3 \\
\Z3x3 & \Pi_e^{-1}Q\end{array} \right],$$
and

\begin{eqnarray*}
\tilde{\mbox{\boldmath $\tau$}}&=&\mbox{\boldmath $\tau$}-\left[\begin{array}{cc} Q & \Z3x3 \\
\Z3x3 & \Pi_e^{-1}Q \end{array} \right]^TK_d \left[\begin{array}{cc} Q & \Z3x3 \\
\Z3x3 & \Pi_e^{-1}Q \end{array} \right] \mbox{\boldmath $\nu$} \\[0.2cm]
&=&\left[\begin{array}{cc} Q & \Z3x3 \\
\Z3x3 & \Pi_e^{-1}Q \end{array} \right]^T \left[\begin{array}{c}
K_p^{r}\tilde{\mbox{\boldmath $\theta$}}+K_i^{r} \mbox{\boldmath $\varphi$}_{\boldsymbol{\theta}}\\
K_p^{t}\tilde{\mathbf{x}}+K_i^{t} \mbox{\boldmath $\varphi$}_{\mathbf{x}}
\end{array}\right]
\end{eqnarray*}

with 

\begin{align*}
\tilde{\mbox{\boldmath $\theta$}} &= \mbox{\boldmath $\theta$}- \mbox{\boldmath $\theta$}_{ref}, 
\hspace{6mm}
\dot{\tilde{\mbox{\boldmath $\theta$}}} = \dot{\mbox{\boldmath $\theta$}} = \Pi_e^{-1}Q\, \mbox{\boldmath $\omega$} ,
\hspace{6mm}
\tilde{\mathbf{x}} = \mathbf{x}-\mathbf{x}_{ref},
\hspace{6mm}
\dot{\mbox{\boldmath $\varphi$}}_{\boldsymbol{\theta}} =\tilde{\mbox{\boldmath $\theta$}},
\hspace{6mm}
\dot{\mbox{\boldmath $\varphi$}}_{\mathbf{x}} =\tilde{\mathbf{x}}.
\end{align*}

\end{Proposition}
\begin{proof}
The proof follows by a direct calculation of the gradient of $H$. 
\end{proof}

The obtained system is completely analog to  \eqref{eq:xiDiff}, and its passivity follows from Proposition~\ref{passivity}.
To obtain a passivity preserving splitting of the vessel model, we can proceed  by splitting $S$ in \eqref{eq:skewMat} as the sum of the two following skew symmetric terms %
{\scriptsize
$$
S_1(\mbox{\boldmath $\xi$}) := \begin{bmatrix} 
0_{3 \times 3} & \widehat{\mathbf{p}} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  0_{3 \times 3} &0_{3 \times 3} \\ 
\widehat{\mathbf{p}}  &\widehat{\mathbf{m}} & 0_{3 \times 3} &0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3}  & 0_{3 \times 3}\\ 
%
 0_{3 \times 3} &  0_{3 \times 3} & -\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3} & 0_{3 \times 3} &0_{3 \times 3} & 0_{3 \times 3}\\
 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  -\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3}  &   0_{3 \times 3} & 0_{3 \times 3}\\
 0_{3 \times 3} & 0_{3 \times 3} &  0_{3 \times 3} &   0_{3 \times 3} &   -\widehat{T^{-1}\mathbf{m}} &  0_{3 \times 3}  & 0_{3 \times 3}\\
 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3}\\
0_{3 \times 3} & 0_{3 \times 3} &  0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} & 0_{3 \times 3}
\end{bmatrix},
$$
%
$$
S_2(\mbox{\boldmath $\xi$}) := \begin{bmatrix} 
0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  0_{3 \times 3} & -Q^T  \\ 
 0_{3 \times 3}&0_{3 \times 3} & 0_{3 \times 3} &0_{3 \times 3} & -\widehat{\mbox{\boldmath $\mu$}} & 0_{3 \times 3}  & 0_{3 \times 3}\\ 
%
 0_{3 \times 3} &  0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &0_{3 \times 3} & 0_{3 \times 3}\\
 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  0_{3 \times 3}& 0_{3 \times 3}  &   0_{3 \times 3} & 0_{3 \times 3}\\
 0_{3 \times 3} & -\widehat{\mbox{\boldmath $\mu$}} &  0_{3 \times 3} &   0_{3 \times 3} &  0_{3 \times 3} &   -\widehat{T^{-1}\mathbf{m}}\,\mathcal{G}  & 0_{3 \times 3}\\
 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & -\mathcal{G}\,\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3} & 0_{3 \times 3}\\
Q  & 0_{3 \times 3} &  0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} & 0_{3 \times 3}
\end{bmatrix} ,
%
$$
}
and then applying an energy-preserving/energy-dissipative integrator on each of the individual flows. The energy in this case is quadratic.  By Proposition~\ref{propositionpassivitysplitting}, %
such a splitting method preserves passivity. In the next section we consider the implementation of this method in a special case, when the splitting leads to two completely integrable flows.

\vspace{1em}





%%%%%%%%
%%%%%%%%%


==> Submission arXiv/Chapters/3_Numerical_solutions.tex <==
%\section{The numerical solution of input-output passive systems with splitting methods} %the marine vessel equations}


%We will here present the numerical approach we use to approximate the solution of
%the marine vessel equations of motion.

%After briefly introducing the relevant splitting methods, we consider a more general system, before moving over to the specific marine vessel %equations.
\subsection{Splitting methods}
\label{numerical}
Consider a general system of first order ODEs where the right hand side vector field admits the splitting

\begin{equation}
\label{eq:split}
\dot{\mathbf{y}} = \mathbf{S_1}(\mathbf{y}) + \mathbf{S_2}(\mathbf{y}).
\end{equation}

We generate a numerical approximation of \eqref{eq:split} by composing the exact flows of $\mathbf{S_1}$ and $\mathbf{S_2}$, computed on time intervals of suitable length, with suitable initial values. Let $\boldsymbol{\Phi}_{h}^{[\mathbf{S_1}]}$ and $\boldsymbol{\Phi}_{h}^{[\mathbf{S_2}]}$ denote, respectively, the exact flow maps of $\mathbf{S_1}$ and $\mathbf{S_2}$. The Lie-Trotter splitting, giving approximations of order $1$, is
\begin{equation}\label{eq:lt}
\mathbf{y}^{j+1} = \boldsymbol{\Phi}_{h}^{[\mathbf{S_2}]}\circ \boldsymbol{\Phi}_{h}^{[\mathbf{S_1}]}
\left(\mathbf{y}^{j}\right),\quad \mathrm{or}\quad \mathbf{y}^{j+1} =\boldsymbol{\Phi}_{h}^{[\mathbf{S_1}]}\circ \boldsymbol{\Phi}_{h}^{[\mathbf{S_2}]} \,
\left(\mathbf{y}^{j}\right).
\end{equation}
An approximation of order 2 is given by the classical Strang splitting scheme as
\begin{equation}\label{eq:s-v0}
\mathbf{y}^{j+1} = \boldsymbol{\Phi}_{h/2}^{[\mathbf{S_1}]}\circ \boldsymbol{\Phi}_{h}^{[\mathbf{S_2}]} \circ\boldsymbol{\Phi}_{h/2}^{[\mathbf{S_1}]}\,
\left(\mathbf{y}^{j}\right),
\end{equation}
or alternatively
\begin{equation}\label{eq:s-v}
\mathbf{y}^{j+1} = \boldsymbol{\Phi}_{h/2}^{[\mathbf{S_2}]}\circ \boldsymbol{\Phi}_{h}^{[\mathbf{S_1}]} \circ\boldsymbol{\Phi}_{h/2}^{[\mathbf{S_2}]}\,
\left(\mathbf{y}^{j}\right).
\end{equation}
%This scheme is known to be symplectic and to
%give a method of order 2.
The two flows $\mathbf{S_1}$ and $\mathbf{S_2}$ can also be combined to obtain splitting
methods of higher order. Specifically, symmetric splitting schemes of the
type %(see \cite{exactcomp})
\begin{equation}
\label{splittinggeneral}
\mathbf{y}^{j+1} = \boldsymbol{\Phi}_{a_1h}^{[\mathbf{S_2}]}\circ \boldsymbol{\Phi}_{b_1h}^{[\mathbf{S_1}]} \circ\boldsymbol{\Phi}_{a_2h}^{[\mathbf{S_2}]}
\circ \cdots \circ \boldsymbol{\Phi}_{a_{m+1}h}^{[\mathbf{S_2}]} \circ \cdots \circ \boldsymbol{\Phi}_{b_1h}^{[\mathbf{S_1}]} \circ \boldsymbol{\Phi}_{a_1h}^{[\mathbf{S_2}]}\,
\left(\mathbf{y}^{j}\right),
\end{equation}
are considered. These are a generalization of the scheme \eqref{eq:s-v}.
%We reproduce t
The Strang splitting can be reproduced from the general formula \eqref{splittinggeneral} by choosing $m=1$, $a_1 = b_1 = 1/2$ and $a_2 = 0$.
%(in the way
%we have presented the scheme above, it is easier to recognize the Strang splitting scheme if
%the coefficients are set to $a_1 = 1/2$, $a_2=0$, and $b_1 = 1/2$).
The coefficients of a $4$th and a $6$th order scheme are reported in Appendix \ref{SplittingCoef}.

% is obtained with the coefficients:
%%Let us first give the coefficients to the fourth order method:
%
%\begin{center}
%\begin{tabular}{lcl}
%$a_1 = 0.0792036964311957$ && $b_1 = 0.209515106613362$ \\
%$a_2 = 0.353172906049774$ && $b_2 = -0.143851773179818$ \\
%$a_3 = -0.0420650803577195$ && $b_3 = \frac{1}{2}-(b_1+b_2)$  \\
%$a_4 = 1-2(a_1+a_2+a_3)$ && \\
%\end{tabular}
%\end{center}

We refer
to \cite{blanes} for other schemes which are used in the numerical experiments.
We remark that the exact flows of $\mathbf{S_1}$ and $\mathbf{S_2}$ can be replaced with suitable high order numerical approximations, while keeping the overall order of the splitting method unchanged.



%\subsection{General case}
%
%Assume a set of ordinary differential equations where the variables can be split into 3 parts  $\mathbf{y}$, $\mathbf{z}$ and $\mathbf{u}$
% 
%\begin{align} 
%\label{eq:simplifiednotation}
%\dot{\mathbf{y}} &= f(\mathbf{y})+G\mathbf{y}+w(\mathbf{z},\mathbf{u}), \nonumber \\
%\dot{\mathbf{z}} &= g(\mathbf{y},\mathbf{z}), \\
%\dot{\mathbf{u}} &= d(\mathbf{z}). \nonumber
%\end{align}
%Here $G$ is a constant matrix while $d$, $f$, $g$ and $w$ are functions, possibly non-linear, of the stated variables.


%We perform the splitting of this system by partitioning the vector field in the following two systems
%\begin{equation}\label{eq:flows1}
%S_1 = \left\{\begin{array}{lcl}\dot{\mathbf{y}} &=& f(\mathbf{y}) \\
%\dot{\mathbf{z}} &=& g(\mathbf{y},\mathbf{z}) \\
%\dot{\mathbf{u}} &=& \mathbf{0}
%\end{array} \right. ,
%\end{equation}

%and

%\begin{equation}\label{eq:flows2}
%S_2 = \left\{\begin{array}{lcl}\dot{\mathbf{y}} &=& G\mathbf{y}+w(\mathbf{z},\mathbf{u})\\
%\dot{\mathbf{z}} &=& \mathbf{0} \\
%\dot{\mathbf{u}} &=& d(\mathbf{z})
%\end{array} \right. .
%\end{equation}

%We notice that in $S_2$, $\mathbf{z}$ is constant. As a consequence $\mbox{\boldmath $\varphi$}_q$ is just a linear function of time. This in turn %means that the equation for $\mathbf{y}$ can be easily solved by the linear variation of constants formula $$\mathbf{y}(\tau)=e^{\tau G}\mathbf{y}_0+%\int_0^\tau e^{(\tau-\sigma)G}(w(\mathbf{z}_0)+\tilde{w}(\mathbf{z}_0)(\mbox{\boldmath $\varphi$}_{q,0}+N\mathbf{z}_0\sigma))\,d\sigma.$$
%This involves the computation of exponentials of $3\times 3$ diagonal matrices.

\subsection{Passivity-preserving splitting  of input-state-output port-Hamiltonian systems}
\label{splittingvessel}

We split the %vessel 
equations \eqref{eq:xiDiff}
%$$
%\dot{\mbox{\boldmath $\xi$}} = S(\mbox{\boldmath $\xi$})\nabla H(\mbox{\boldmath $\xi$}) -G\left(D(\mbox{\boldmath $\xi$})\mbox{\boldmath $\nu$} - \mbox{\boldmath $\tau$}\right),
%$$
by splitting the skew symmetric matrix $S(\mbox{\boldmath $\xi$})$ into the sum of two skew-symmetric terms $S(\mbox{\boldmath $\xi$})=S_1(\mbox{\boldmath $\xi$})+S_2(\mbox{\boldmath $\xi$})$.
% for example  as follows %of two skew symmetric terms where
%into two completely integrable subsystems, and make some remarks on their numerical solution using splitting methods.
%The vessel equations can subbe written as an autonomous system of equations. We partition the variables in three subsets:
%$$\mathbf{y}=[\mathbf{m},\mathbf{v}],\quad \mathbf{z}=[\mathbbm{q},\mathbf{x},\mbox{\boldmath $\varphi$}_x], \quad  \mathbf{u} = \mbox{\boldmath $%%%%\varphi$}_q$$
%Notice that the splitting of the vessel equations which we have proposed in section~\ref{splittingvessel} corresponds to the choice
%{\scriptsize
%$$
%S_1(\mbox{\boldmath $\xi$}) := \begin{bmatrix} 
%0_{3 \times 3} & \widehat{\mathbf{p}} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  0_{3 \times 3} &0_{3 \times 3} \\ 
%\widehat{\mathbf{p}}  &\widehat{\mathbf{m}} & 0_{3 \times 3} &0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3}  & 0_{3 \times 3}\\ 
%%0_{3 \times 3} & -m_v\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  0_{3 \times 3} &-Q^T \\ 
% 0_{3 \times 3} &  0_{3 \times 3} & -\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3} & 0_{3 \times 3} &0_{3 \times 3} & 0_{3 \times 3}\\
% 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  -\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3}  &   0_{3 \times 3} & 0_{3 \times 3}\\
% 0_{3 \times 3} & 0_{3 \times 3} &  0_{3 \times 3} &   0_{3 \times 3} &   -\widehat{T^{-1}\mathbf{m}} &  0_{3 \times 3}  & 0_{3 \times 3}\\
% 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3}\\
%0_{3 \times 3} & 0_{3 \times 3} &  0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} & 0_{3 \times 3}
%\end{bmatrix},
%$$
%%$$
%%S_1(\mbox{\boldmath $\xi$}) := \begin{bmatrix} 
%%\widehat{\mathbf{m}} & 0_{3 \times 3} & 0_{3 \times 3} &0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &   0_{3 \times 3}\\ 
%%0_{3 \times 3} & -m_v\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &   0_{3 \times 3}\\ 
%% 0_{3 \times 3} &  0_{3 \times 3} & -\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3} & 0_{3 \times 3} &0_{3 \times 3} &   0_{3 \times 3} \\
%% 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  -\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3}  &   0_{3 \times 3} &   0_{3 \times 3}\\
%%0_{3 \times 3} &  0_{3 \times 3} &  0_{3 \times 3} &   0_{3 \times 3} &   -\widehat{T^{-1}\mathbf{m}}&   0_{3 \times 3} &   0_{3 \times 3} \\
%%0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3}\\
%%0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3}\\
%%\end{bmatrix}, 
%%$$
%$$
%S_2(\mbox{\boldmath $\xi$}) := \begin{bmatrix} 
%0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  0_{3 \times 3} & -Q^T  \\ 
% 0_{3 \times 3}&0_{3 \times 3} & 0_{3 \times 3} &0_{3 \times 3} & -\widehat{\mbox{\boldmath $\mu$}} & 0_{3 \times 3}  & 0_{3 \times 3}\\ 
%%0_{3 \times 3} & -m_v\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  0_{3 \times 3} &-Q^T \\ 
% 0_{3 \times 3} &  0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &0_{3 \times 3} & 0_{3 \times 3}\\
% 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  0_{3 \times 3}& 0_{3 \times 3}  &   0_{3 \times 3} & 0_{3 \times 3}\\
% 0_{3 \times 3} & -\widehat{\mbox{\boldmath $\mu$}} &  0_{3 \times 3} &   0_{3 \times 3} &  0_{3 \times 3} &   -\widehat{T^{-1}\mathbf{m}}\,\mathcal{G}  & 0_{3 \times 3}\\
% 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & -\mathcal{G}\,\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3} & 0_{3 \times 3}\\
%Q  & 0_{3 \times 3} &  0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} & 0_{3 \times 3}
%\end{bmatrix} .
%%S_2(\mbox{\boldmath $\xi$}) := \begin{bmatrix} 
%%0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &0_{3 \times 3} & \widehat{\mbox{\boldmath $\mu$}}  & 0_{3 \times 3} &   0_{3 \times 3}\\ 
%%0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &   0_{3 \times 3} & -Q^T  \\ 
%% 0_{3 \times 3} &  0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &0_{3 \times 3} &   0_{3 \times 3}\\
%% 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3}& 0_{3 \times 3}  &   0_{3 \times 3} &   0_{3 \times 3}\\
%%\widehat{\mbox{\boldmath $\mu$}}  &  0_{3 \times 3} &  0_{3 \times 3} &   0_{3 \times 3} &    0_{3 \times 3} & \widehat{T^{-1}\mathbf{m}}\,\mathcal{G}  &   0_{3 \times 3}\\
%% 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & \mathcal{G}\,\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3} & 0_{3 \times 3}\\
%%0_{3 \times 3} & Q & 0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3}
%%\end{bmatrix}.
%$$
%}
%


\begin{Proposition}
\label{propositionpassivitysplitting}
The order $1$  splitting method \eqref{eq:lt}, when applied to the flows of the two systems 
\begin{equation}
\label{splitting}
\left\{\begin{array}{lcl}
\dot{\mbox{\boldmath $\xi$}}&=&S_1(\mbox{\boldmath $\xi$})\nabla H(\mbox{\boldmath $\xi$})\\
\mbox{\boldmath $\xi$}(0)&=&\mbox{\boldmath $\xi$}_0,
\end{array}\right.\, \mathrm{on}\,\, [0,h],\quad
\left\{\begin{array}{lcl}
\dot{\tilde{\mbox{\boldmath $\xi$}}}&=&S_2(\tilde{\mbox{\boldmath $\xi$}})\nabla H(\tilde{\mbox{\boldmath $\xi$}})-G\left(D\tilde{\mbox{\boldmath $\nu$}} - \mbox{\boldmath $\tau$}\right)\\
\tilde{\mbox{\boldmath $\xi$}}(0)&=&\tilde{\mbox{\boldmath $\xi$}}_0,
\end{array}\right.\, \mathrm{on}\,\, [0,h],
\end{equation}
and with $\tilde{\mbox{\boldmath $\xi$}}_0=\mbox{\boldmath $\xi$}(h)$, is input-output passive with input $\mbox{\boldmath $\tau$}$ and output $\tilde{\mbox{\boldmath $\nu$}}=G\,\nabla H(\tilde{\mbox{\boldmath $\xi$}})$.
\end{Proposition}

\begin{proof}
We want to prove that \eqref{passivity1} holds with $V=H$. We have
\begin{eqnarray*}
H(\tilde{\mbox{\boldmath $\xi$}}(h))-H(\mbox{\boldmath $\xi$}_0)&=& H(\tilde{\mbox{\boldmath $\xi$}}(h))-H(\tilde{\mbox{\boldmath $\xi$}}_0)+H(\mbox{\boldmath $\xi$}(h))-H(\mbox{\boldmath $\xi$}_0)\\
&=& \int_0^h\nabla H(\tilde{\mbox{\boldmath $\xi$}}(s))^T\dot{\tilde{\mbox{\boldmath $\xi$}}}(s)\,ds +\int_0^h\nabla H(\mbox{\boldmath $\xi$}(s))^T\dot{\mbox{\boldmath $\xi$}}(s)\,ds \\
&=&\int_0^h\nabla H(\tilde{\mbox{\boldmath $\xi$}}(s))^T\left(S_2(\tilde{\mbox{\boldmath $\xi$}})\nabla H(\tilde{\mbox{\boldmath $\xi$}})-G\left(D\tilde{\mbox{\boldmath $\nu$}}-\mbox{\boldmath $\tau$}\right)\right)\,ds +\\
& &+\int_0^h\nabla H(\mbox{\boldmath $\xi$}(s))^TS_1(\mbox{\boldmath $\xi$}(s))\nabla H(\mbox{\boldmath $\xi$}(s))\,ds, \\
\end{eqnarray*}
and by using the skew-symmetry of $S_1$ and $S_2$ we get finally
\begin{eqnarray*}
H(\tilde{\mbox{\boldmath $\xi$}}(h))-H(\mbox{\boldmath $\xi$}_0)&=&-\int_0^h\nabla H(\tilde{\mbox{\boldmath $\xi$}}(s))^TG\left(D\tilde{\mbox{\boldmath $\nu$}}-\mbox{\boldmath $\tau$}\right)\,ds\\
&=&-\int_0^h \tilde{\mbox{\boldmath $\nu$}}^T\left(D\tilde{\mbox{\boldmath $\nu$}}-\mbox{\boldmath $\tau$}\right)\,ds.
\end{eqnarray*}
Notice that the order of composition of the flows is immaterial.
If we now choose $V=H$, $\mathbf{y}=\tilde{\mbox{\boldmath $\xi$}}$, $\mathbf{u}=\mbox{\boldmath $\tau$}$ and 
$\boldsymbol{\zeta}=\tilde{\mbox{\boldmath $\nu$}}$, then it follows that the composition of the flows of the systems \eqref{splitting} satisfies Definition \ref{defpass} with  $g(\mathbf{y})=\tilde{\mbox{\boldmath $\nu$}}^T \, D \tilde{\mbox{\boldmath $\nu$}}$ and output $\tilde{\mbox{\boldmath $\nu$}}$.
%$\mathbf{h}(\mathbf{y}) = [(T^{-1}\mathbf{m})^T,
%(m_v^{-1}\mathbf{p})^T]^T$. 
%Thus the system is passive. The requirement $g(\mathbf{y}) \geq 0$ is fulfilled because the matrix $D$ is positive-definite. 
\end{proof}

\begin{Remark} The passivity result proved in Proposition~\ref{propositionpassivitysplitting} for the simple order $1$ splitting of two flows, generalises to
the order $1$ splitting and composition of $m$ flows arising from writing $S$ as a sum of $m$ skew-symmetric terms, $S(\mbox{\boldmath $\xi$})=\sum_{i=1}^mS_i (\mbox{\boldmath $\xi$})$. This  splitting method is a direct generalisation of  \eqref{eq:lt}.
\end{Remark}



\begin{Remark} The passivity result proved in Proposition~\ref{propositionpassivitysplitting} for the simple splitting method of order $1$ generalises easily to the Strang splitting given by \eqref{eq:s-v0} and \eqref{eq:s-v}. Note however, that it is crucial in the proof that the coefficients of the splitting method are real and positive. There are no splitting methods of order higher than $2$ with this property, \cite{blanesComplexcoeff}.  But there exist splitting methods of order greater than or equal to $3$  with complex coefficients which have positive real part, see for instance \cite{blanesComplexcoeff}. The construction and implementation of passivity preserving splitting methods of higher order for rigid body dynamics using complex coefficients is not pursued here, but can be an interesting subject for future investigations. 
\end{Remark} 


\begin{Remark}
If the splitting method used for the integration has order $p$, then it is possible to replace the exact flows of the two subsystems with approximate numerical flows of order $p$ without compromising the order of the method. If the corresponding numerical flows are energy-preserving for the first system of the splitting, and energy-dissipative for the second system, then the overall splitting method with positive coefficients remains input-output passive. Methods with such preservation/dissipation properties  
can be found among implicit Runge-Kutta schemes for polynomial vector fields \cite{celledoni09epr}, and among discrete gradient methods and their generalizations for general vector fields \cite{mclachlanDG}, \cite{hairer}.
\end{Remark} 

We next consider a simplified system for which the proposed splitting method always dissipates the total energy independently of the sign of the (real) coefficients of the splitting method.
Specifically, we consider the system
\begin{equation}
\label{system2}
\dot{\mbox{\boldmath $\xi$}} = (S(\mbox{\boldmath $\xi$})-D(\mbox{\boldmath $\xi$}) )\nabla H(\mbox{\boldmath $\xi$}) ,
\end{equation}
with $S\in\mathbf{R}^{m\times m}$ skew symmetric, $D\in\mathbf{R}^{m\times m}$ symmetric and positive definite. Note that the system \eqref{eq:xiDiff} can be rewritten in this form under the assumption that $\mbox{\boldmath $\tau$}=-KG^T\nabla H(\mbox{\boldmath $\xi$})$ with $K\in\mathbf{R}^{p\times p}$ symmetric and positive semi-definite. Let $H$ be a quadratic energy function $ H(\mbox{\boldmath $\xi$})=\mbox{\boldmath $\xi$}^T\tilde{H} \,\mbox{\boldmath $\xi$}$, with $\tilde{H}\in\mathbf{R}^{m\times m}$ symmetric and positive definite. We can then define the energy norm
$$\|\mbox{\boldmath $\xi$}\|_{H}:=\sqrt{\mbox{\boldmath $\xi$}^T\tilde{H} \,\mbox{\boldmath $\xi$}},$$ associated with the inner product $\langle \cdot , \cdot\rangle_H:= \langle \cdot , \tilde{H} \cdot\rangle$. 
\begin{Lemma}\label{lemma1}
System \eqref{system2} satisfies
\begin{equation}
\label{onesidedLipshitzconstant}
\langle (S(\mbox{\boldmath $\xi$})-D(\mbox{\boldmath $\xi$}) )\nabla H(\mbox{\boldmath $\xi$}) , \mbox{\boldmath $\xi$} \rangle_H\le-2\sigma_{\min} \, \|\mbox{\boldmath $\xi$}\|_H^2
\end{equation}
and
\begin{equation}
\label{onesidedLipshitzconstantminus}
\langle -(S(\mbox{\boldmath $\xi$})-D(\mbox{\boldmath $\xi$}) )\nabla H(\mbox{\boldmath $\xi$}) , \mbox{\boldmath $\xi$} \rangle_H\le 2\sigma_{\max} \, \|\mbox{\boldmath $\xi$}\|_H^2
\end{equation}

with $\sigma_{\max}\ge\sigma_{\min}> 0$.
\end{Lemma}
\begin{proof}
We have $\nabla H =2\,\tilde{H} \, \mbox{\boldmath $\xi$}$, so
\begin{equation}
\label{eq:innprod}
\langle (S(\mbox{\boldmath $\xi$})-D(\mbox{\boldmath $\xi$}) )\nabla H(\mbox{\boldmath $\xi$}) , \mbox{\boldmath $\xi$} \rangle_H = -2\mbox{\boldmath $\xi$}^T\tilde{H}(S(\mbox{\boldmath $\xi$})+D(\mbox{\boldmath $\xi$}) )\tilde{H} \, \mbox{\boldmath $\xi$}
=-2\mbox{\boldmath $\xi$}^T\tilde{H}D\tilde{H}\mbox{\boldmath $\xi$},
\end{equation}
%and we have
%$$\mbox{\boldmath $\xi$}^T\tilde{H}D\tilde{H}\mbox{\boldmath $\xi$} = (\tilde{H}^{\frac{1}{2}}\mbox{\boldmath $\xi$})^T(\tilde{H}^{\frac{1}{2}}D\tilde{H}^{\frac{1}{2}})(\tilde{H}^{\frac{1}{2}}\mbox{\boldmath $\xi$})$$
%so that, i
If $\sigma_{\max} > 0$ and $\sigma_{\min} > 0$ are the maximum and minimum eigenvalue of $\tilde{H}^{\frac{1}{2}}D\tilde{H}^{\frac{1}{2}}$, we have
%$$\sigma_{\min} \|\mbox{\boldmath $\xi$}\|^2_H=\sigma_{\min}\|\tilde{H}^{\frac{1}{2}} \mbox{\boldmath $\xi$}\|_2^2\le 
%\mbox{\boldmath $\xi$}^T\tilde{H}D\tilde{H}\mbox{\boldmath $\xi$}
%% \mbox{\boldmath $\xi$}^T\tilde{H}^{\frac{1}{2}}(\tilde{H}^{\frac{1}{2}}D\tilde{H}^{\frac{1}{2}})\tilde{H}^{\frac{1}{2}}\mbox{\boldmath $\xi$}
%\le \sigma_{\max} 
%\|\tilde{H}^{\frac{1}{2}} \mbox{\boldmath $\xi$}\|^2_2=\sigma_{\max} \|\mbox{\boldmath $\xi$}\|^2_H.$$
\begin{equation}
\label{eq:eigenv}
\sigma_{\min} \|\mbox{\boldmath $\xi$}\|^2_H=\sigma_{\min}\|\tilde{H}^{\frac{1}{2}} \mbox{\boldmath $\xi$}\|_2^2\le 
\mbox{\boldmath $\xi$}^T\tilde{H}D\tilde{H}\mbox{\boldmath $\xi$}
% \mbox{\boldmath $\xi$}^T\tilde{H}^{\frac{1}{2}}(\tilde{H}^{\frac{1}{2}}D\tilde{H}^{\frac{1}{2}})\tilde{H}^{\frac{1}{2}}\mbox{\boldmath $\xi$}
\le \sigma_{\max} 
\|\tilde{H}^{\frac{1}{2}} \mbox{\boldmath $\xi$}\|^2_2=\sigma_{\max} \|\mbox{\boldmath $\xi$}\|^2_H.
%-2\sigma_{\max} \|\mbox{\boldmath $\xi$}\|^2_H\le -2\mbox{\boldmath $\xi$}^T\tilde{H}D\tilde{H}\mbox{\boldmath $\xi$}\le -2\sigma_{\min} \|\mbox{\boldmath $\xi$}\|^2_H, 
\end{equation}
% from the fact that there is a constant $\sigma\ge 0$ such that

Notice that, by Sylvester's law of inertia,  $\tilde{H}^{\frac{1}{2}}D\tilde{H}^{\frac{1}{2}}$ is symmetric positive definite since $D$ and $\tilde{H}$ are.  From \eqref{eq:innprod} and \eqref{eq:eigenv}, \eqref{onesidedLipshitzconstant} and \eqref{onesidedLipshitzconstantminus} follow.
%, and $\sigma_{\min}$ can be taken to be the smallest eigenvalue of $\tilde{H}^{\frac{1}{2}}D\tilde{H}^{\frac{1}{2}}$.
\end{proof}
The following Lemma is an adaptation of the results of \cite[p.180]{hairer91sod}.
\begin{Lemma} \label{lemma2} 
Assume $\sigma_{\max}\ge\sigma_{\min} > 0$ and \eqref{onesidedLipshitzconstant} and \eqref{onesidedLipshitzconstantminus} hold. %or \eqref{onesidedLipshitzconstant} holds for $\sigma_{\max}\ge 0$ 
Then for $t\ge 0$ along continuous solutions $\mbox{\boldmath $\xi$}$ of \eqref{system2} we have
\begin{equation}
\label{dissipationH}
H(\mbox{\boldmath $\xi$}(t))\le e^{-4t\sigma_{\min}} H(\mbox{\boldmath $\xi$}(0));
\end{equation}
for $t \le 0$ along continuous solutions $\mbox{\boldmath $\xi$}$ of \eqref{system2} we have
\begin{equation}
\label{propagationH}
H(\mbox{\boldmath $\xi$}(t))\le e^{-4t\sigma_{\max}} H(\mbox{\boldmath $\xi$}(0)).
\end{equation}
\end{Lemma}
\begin{proof}
We have
$$\frac{d H(\mbox{\boldmath $\xi$}(t))}{dt}=\nabla H(\mbox{\boldmath $\xi$})^T\dot{\mbox{\boldmath $\xi$}}(t)=2\langle (S(\mbox{\boldmath $\xi$})-D(\mbox{\boldmath $\xi$}) )\nabla H(\mbox{\boldmath $\xi$}) , \mbox{\boldmath $\xi$} \rangle_H,$$
for $t\ge 0$.
From \eqref{onesidedLipshitzconstant} %Lemma~\ref{lemma1} 
we then get
$$\frac{d H(\mbox{\boldmath $\xi$}(t))}{dt}\le-4\sigma_{\min} H(\mbox{\boldmath $\xi$}(t)),
$$
$H(t)=H(\mbox{\boldmath $\xi$}(t))$ is a continuous function of $t$ if $\mbox{\boldmath $\xi$}(t)$ is. Integrating the obtained differential inequality we get \eqref{dissipationH}.

Notice that integrating \eqref{system2} with negative time corresponds to solving 
$$\dot{\mbox{\boldmath $\xi$}} = -(S(\mbox{\boldmath $\xi$})-D(\mbox{\boldmath $\xi$}) )
\nabla H(\mbox{\boldmath $\xi$} ) $$ for $t\ge 0$, so differentiating $H(\mbox{\boldmath $\xi$}(t))$ with respect to $t$ and using \eqref{onesidedLipshitzconstantminus}, we arrive in this case \eqref{propagationH}. %in the proof of 
\end{proof}

\vskip0.2cm


\vskip0.2cm
Assume $S=S_1+S_2$ with both $S_1$ and $S_2$ skew-symmetric. In what follows we give a sufficient condition for \eqref{splittinggeneral} to be energy dissipative even when the coefficients of the splitting method are real and both positive and negative.
\begin{Proposition}
\label{propositionpassivitysplittingquadraticenergy}
The splitting method \eqref{splittinggeneral} of order $p\ge 1$ given by composing the flows  
{\small
\begin{equation}
\mathbf{S}_1: \left\{\begin{array}{lcl}
\dot{\mbox{\boldmath $\xi$}}&=&S_1(\mbox{\boldmath $\xi$})\nabla H(\mbox{\boldmath $\xi$})\\
\mbox{\boldmath $\xi$}(0)&=&\mbox{\boldmath $\xi$}_0
\end{array}\right.\, \mathrm{on}\,\, [0,h],\quad
\mathbf{S}_2: \left\{\begin{array}{lcl}
\dot{\tilde{\mbox{\boldmath $\xi$}}}&=&(S_2(\tilde{\mbox{\boldmath $\xi$}})  - D ( \tilde{\mbox{\boldmath $\xi$}}) )\nabla H(\tilde{\mbox{\boldmath $\xi$}})\\
\tilde{\mbox{\boldmath $\xi$}}(0)&=&\tilde{\mbox{\boldmath $\xi$}}_0
\end{array}\right.\, \mathrm{on}\,\, [0,h],
\end{equation}
}
and with $\tilde{\mbox{\boldmath $\xi$}}_0=\mbox{\boldmath $\xi$}(h)$, is energy dissipative if
\begin{equation}
\label{eq:condition}
2\,\sum_{i=1}^m\mu_ia_i+\mu_{m+1}a_{m+1}\ge 0, \quad \mu_i:=\left\{\begin{array}{ccc}
\sigma_{\min} &  \mathrm{if} & a_i>0,\\
\sigma_{\max} & \mathrm{if} & a_i <0,
\end{array}\right.
\end{equation}
with $\sigma_{\max}$ and $\sigma_{\min}$ the maximum and minimum eigenvalue of $\tilde{H}^{\frac{1}{2}}D\tilde{H}^{\frac{1}{2}}$.
  %input-output passive with input $\mbox{\boldmath $\tau$}$ and output $\tilde{\mbox{\boldmath $\nu$}}$.
\end{Proposition}
\begin{proof}
By the order $1$ conditions of the splitting method \cite[sec. III.3.4]{gni06hairer} we have
$$2\,\sum_{i=1}^ma_m+a_{m+1}=1,\quad    2\sum_{i=1}^mb_i=1.$$
Consider 
$$\mu_i:=\left\{\begin{array}{ccc}
\sigma_{\min} &  \mathrm{if} & a_i>0,\\
\sigma_{\max} & \mathrm{if} & a_i <0.
\end{array}\right.
$$
For the solution, $\tilde{\mbox{\boldmath $\xi$}}(t)$, of the system $\mathbf{S}_2$, we have from Lemma~\ref{lemma2} that on the time interval $[0,a_ih]$, 
$$H(\tilde{\mbox{\boldmath $\xi$}}(a_ih))%=\|\tilde{\mbox{\boldmath $\xi$}}(a_ih)\|_{H}^2
\le %e^{-2\mu_ia_ih}\, \|\tilde{\mbox{\boldmath $\xi$}}(0)\|_{H}^2=
e^{-4\mu_ia_ih}\,H(\tilde{\mbox{\boldmath $\xi$}}(0)).$$
%for $a_i > 0$ %, by Lemma~\ref{lemma2}
%$$H(\tilde{\mbox{\boldmath $\xi$}}(a_ih))=\|\tilde{\mbox{\boldmath $\xi$}}(a_ih)\|_{H}^2\le e^{-2\sigma_{\min}(a_ih)}\, \|\tilde{\mbox{\boldmath $\xi$}}(0)\|_{H}^2=e^{-2\sigma_{\min}(a_ih)}\,H(\tilde{\mbox{\boldmath $\xi$}}(0)).$$
%%where $\mu\ge 0$ and $\frac{\mu}{2}$ is the minimum eigenvalue of $\tilde{H}^{\frac{1}{2}}D\tilde{H}^{\frac{1}{2}}$.
%%plays the role of the constant $\sigma$ of 
%Similarly on
%$[0,a_jh]$, $a_j < 0$,
%$$H(\tilde{\mbox{\boldmath $\xi$}}(a_jh))=\|\tilde{\mbox{\boldmath $\xi$}}(a_jh)\|_{H}^2\le e^{-2\sigma_{\max}(a_jh)}\, \|\tilde{\mbox{\boldmath $\xi$}}(0)\|_{H}^2=e^{-2\sigma_{\max}(a_jh)}\,H(\tilde{\mbox{\boldmath $\xi$}}(0)).$$
%%where $\nu\ge 0$ and $\frac{\nu}{2}$ is the maximum eigenvalue of $\tilde{H}^{\frac{1}{2}}D\tilde{H}^{\frac{1}{2}}$.
% %is the one-sided Lipshitz constant of $\mathbf{S}_2$, $M$ is less than or equal to zero since $D$ is positive semi-definite \cite[p.180]{hairer91sod}. 
For the solution $\mbox{\boldmath $\xi$}(t)$ of  $\mathbf{S}_1$ on $[0,b_ih]$, we have
$$H(\mbox{\boldmath $\xi$}(b_ih))=%\|\mbox{\boldmath $\xi$}(b_ih)\|_H^2=\|\mbox{\boldmath $\xi$}(0)\|_H^2=
H(\mbox{\boldmath $\xi$}( 0)).$$
Using \eqref{splittinggeneral} and the above inequalities we have
$$H(\mbox{\boldmath $\xi$}^{j+1})\le e^{-4\mu_1 a_1h}e^{-4\mu_2 a_2h}\cdots e^{-4\mu_{m+1} a_{m+1}h}\cdots e^{-4\mu_2 a_2h} e^{-4\mu_1 a_1h}\,   H(\mbox{\boldmath $\xi$}^{j}), %   \|\mbox{\boldmath $\xi$}^{j}\|_H^2,
$$
%where
%$$\mu_i:=\left\{\begin{array}{ccc}
%\sigma_{\min} &  \mathrm{if} & a_i>0,\\
%\sigma_{\max} & \mathrm{if} & a_i <0,
%\end{array}\right.
%$$
 %$\mu_i$ is either the maximum or the minimum eigenvalue of $\tilde{H}^{\frac{1}{2}}D\tilde{H}^{\frac{1}{2}}$ depending on $a_i$ being positive or negative,
and so
$$H(\mbox{\boldmath $\xi$}^{j+1})\le e^{- 4(2\sum_{i=1}^m\mu_ia_i+\mu_{m+1}a_{m+1})}H(\mbox{\boldmath $\xi$}^{j})\le H(\mbox{\boldmath $\xi$}^{j}),$$
if \eqref{eq:condition} is satisfied. %which concludes the proof.
\end{proof}
%Notice that this sufficient condition is mostly useful when $\tilde{H}$ is symmetric positive definite and $\sigma_{\min}>0$, else if $\sigma_{\min}=0$ \eqref{eq:condition} cannot be satisfied.

The coefficients of the method of order four used in our numerical experiments are given in Appendix~\ref{SplittingCoef}. For this method we obtain that condition \eqref{eq:condition} is satisfied  when 
$\frac{\sigma_{\max}}{\sigma_{\min}}\le \frac{2(a_1+a_2)+a_4}{-2a_3}\approx 12$; and interchanging the role of $\mathbf{S}_1$ and $\mathbf{S}_2$, we obtain instead the condition  $\frac{\sigma_{\max}}{\sigma_{\min}}\le \frac{(b_1+b_2)}{-b_3}\approx 4.5$. 

\input{Chapters/2_Vessel_model}



\subsection{Implementation}
\label{implementation}


In the numerical experiments, and in this section, we will consider the case when the mass matrix has the form  \eqref{MRB}. This occurs for example  when the added mass is zero, i.e. $M_A=O$, or when $M_A$ has the same diagonal structure as $M_{RB}$. We will also assume the damping matrix $D$ to be constant. 
As a consequence the term $\mathbf{p}\times \mathbf{v}$ in the equation for the angular momentum is zero (because $\mathbf{p}$ and $\mathbf{v}$ are parallel). For this reason the matrix $S$ can be modified to have a skew symmetric diagonal block $-\widehat{\mbox{\boldmath $\omega$}}$ in the upper left diagonal corner, while both off diagonal blocks of the type $\hat{\mathbf{p}}$ disappear.
The equations \eqref{eq:vessel} simplify and become
\begin{equation}\label{eq:vflows}
\begin{aligned}
\dot{\mathbf{p}} &=-\widehat{\mbox{\boldmath $\omega$}}\,\mathbf{p} -\left(D_t\mathbf{v}+Q^T\mathcal{A}\mathbf{x}-\mbox{\boldmath $\tau$}_t\right), \\
\dot{\mathbf{m}} &= -\widehat{\mbox{\boldmath $\omega$}} \,\mathbf{m} - \left(D_r\mbox{\boldmath $\omega$}+\widehat{\mbox{\boldmath $\mu$}}\,\mathbf{q}_3-\mbox{\boldmath $\tau$}_r\right), \\
\dot{Q}&=Q\,\widehat{\mbox{\boldmath $\omega$}},\\
\dot{\mbox{\boldmath $\mu$}}&= -\mathcal{G}\,\widehat{\mbox{\boldmath $\omega$}}\, \mathbf{q}_3,\\
\dot{\mathbf{x}} &= Q\,\mathbf{v},\\
\dot{\mbox{\boldmath $\varphi$}}_{\boldsymbol{\theta}}&=\tilde{\mbox{\boldmath $\theta$}}, \\
\dot{\mbox{\boldmath $\varphi$}}_{\mathbf{x}}&=\tilde{\mathbf{x}}.
\end{aligned} 
\end{equation}
%with in addition the equations $\dot{\mbox{\boldmath $\varphi$}}_{\boldsymbol{\theta}}=\tilde{\mbox{\boldmath $\theta$}},$ and $\dot{\mbox{\boldmath $\varphi$}}_{\mathbf{x}}=\tilde{\mathbf{x}}$ when $K_i^r$ and $K_i^t$ are non zero.
This case is particularly interesting because it is possible to split $S$ as the sum of two skew symmetric terms $S=S_1+S_2$ while obtaining two completely integrable flows for which explicit solutions can be found. The system $\mathbf{S_1}$, arising from $S_1$, is a free-rigid body flow, as in the more general case of the previous section. Conversely, we will see that the system $\mathbf{S_2}$, arising from $S_2$, is linear and can be integrated exactly using the variation of constants formula. Proposition~\ref{propositionpassivitysplitting} applies directly to this case. In the more general case discrete gradient methods and their higher order generalisations, see  \cite{mclachlanDG} and \cite{hairer}, can be applied to solve $\mathbf{S_2}$.

%The splitting method also in this case should arise from the splitting of the skew symmetric matrix $S=S_1+S_2$, but the two skew symmetric matrices $S_1$ are slightly modified so that the second part of the splitting is a linear equation which can be integrated exactly using the variation of constants formula.

In what follows, regarding notation, we reparametrize time using $\gamma$, such that $\gamma = 0$ represents the current starting point. We also use the convention that index $0$ for a variable, e.g. $\mathbf{x}_0$, denotes the current initial value (at $\gamma = 0$).
\subsubsection{System $\mathbf{S_1}$: Free-rigid body integration}



The system $\mathbf{S_1}$  amounts to a system of free rigid body equations
\begin{equation}\label{eq:vflows1}
\mathbf{S_1} = \left\{\begin{aligned}
\dot{\mathbf{p}} &=-\widehat{\mbox{\boldmath $\omega$}}\,\mathbf{p}, \\
\dot{\mathbf{m}} &= \mathbf{m} \times \mbox{\boldmath $\omega$}, \\
\dot{Q}&=Q\,\widehat{\mbox{\boldmath $\omega$}},\\
\dot{\mbox{\boldmath $\mu$}}&=\mathbf{0},\\
\dot{\mathbf{x}} &= \mathbf{0}, \\ %Q\,\mathbf{v},\\
\dot{\mbox{\boldmath $\varphi$}}_{\boldsymbol{\theta}}&=\mathbf{0}, \\
\dot{\mbox{\boldmath $\varphi$}}_{\mathbf{x}}&=\mathbf{0}.%\tilde{\mathbf{x}}.
\end{aligned} \right. 
\end{equation}
This system is completely integrable. To integrate these equations we employ techniques developed in \cite{celledoni06ets} and \cite{celledoni08tec}. 

%Notice that compared to the splitting of section~\ref{splittingvessel}, $\dot{\mathbf{x}}=\mathbf{0}$ and correspondingly the term depending on $Q$ in the first equation has been moved to the system $\mathbf{S_2}$, while the term $\widehat{\mbox{\boldmath $\omega$}}\mathbf{p}$ has been moved from $\mathbf{S_2}$ to $\mathbf{S_1}$. These are changes which do not affect the integrability of $\mathbf{S_1}$, and the implementation details given in this section are valid also for $\mathbf{S_1}$ as given section~\ref{splittingvessel}.

$\mathbf{S_1}$ is integrated several times on some interval  $[0,\alpha h]$ as a part of the splitting methods, with $h$ being the step size of integration and $\alpha=a_i$, $i=1,\dots , m+1$, i.e. one of the coefficients of the splitting method. We observe that $\dot{\mbox{\boldmath $\omega$}}$ and $\dot{Q}$  do not depend on $\mathbf{v}$ and $\mathbf{x}$. As $\mbox{\boldmath $\omega$}$ can also be computed independently of $Q$, we proceed as follows. We first compute $\mbox{\boldmath $\omega$}$ using explicit formulae based on Jacobi elliptic functions, see \cite{celledoni08tec} Proposition 2.1. Then using $\mbox{\boldmath $\omega$}$, we solve numerically the equation for $Q$ in \eqref{eq:vflows1} using the Magnus series expansion. For a method of order $2$ the computed approximation for $Q$ is
$$
Q^{[2]}=Q_0\exp\left(h\, \widehat{ \mbox{\boldmath $\omega$}^{(\frac{1}{2})} }\right),
$$
with $\mbox{\boldmath $\omega$}^{(\frac{1}{2})}=\mbox{\boldmath $\omega$}(\frac{\alpha}{2h})$.
The two approximations of order $4$ and $6$ require the computation of commutators, and the use of quadrature. They give the approximations:
{\small
$$
Q^{[4]}=Q_0\exp\left(\alpha_1-\frac{1}{12}[\alpha_1,\alpha_2]\right),\quad \alpha_1:=\frac{h}{2}(\widehat{\mbox{\boldmath $\omega$}(c_1h)}+\widehat{\mbox{\boldmath $\omega$}(c_2h)}),\quad \alpha_2:=\sqrt{3}h(\widehat{\mbox{\boldmath $\omega$}(c_2h)}-\widehat{\mbox{\boldmath $\omega$}(c_1h)}),
$$
}
with $c_1=\frac{1}{2}-\frac{\sqrt{3}}{6}$ $c_2=\frac{1}{2}+\frac{\sqrt{3}}{6}$; and
$$
Q^{[6]}=Q_0\exp\left(\alpha_1+\frac{1}{12}\alpha_3+\frac{1}{240}[-20\alpha_1-\alpha_3+s_1,\alpha_2+r_1]\right),$$
where
$$s_1:=[\alpha_1,\alpha_2],\quad r_1=-\frac{1}{60}[\alpha_1,2\alpha_3+s_1],$$
and
{\small
$$ \alpha_1:=h\widehat{\mbox{\boldmath $\omega$}(c_2h)},\quad \alpha_2:= \frac{\sqrt{15}h}{3}(\widehat{\mbox{\boldmath $\omega$}(c_3h)}-\widehat{\mbox{\boldmath $\omega$}(c_1h)}),\quad \alpha_3:=\frac{10h}{3}(\widehat{\mbox{\boldmath $\omega$}(c_3h)}-2\widehat{\mbox{\boldmath $\omega$}(c_2h)})+\widehat{\mbox{\boldmath $\omega$}(c_1h)}),
$$
}
with $c_1=\frac{1}{2}-\frac{\sqrt{15}}{10}$, $c_2=\frac{1}{2}$ and $c_3=\frac{1}{2}+\frac{\sqrt{15}}{10}$.
See also \cite{celledoni06ets}, \cite{gustavson} for details. This method will be referred to as the Magnus method. It was shown in  \cite{blanes02} that this method requires a minimal number of commutators. One can truncate the Magnus expansion to arbitrary high order. Here we have implemented this method to order 2, 4, and 6, and combined it with splittings of the same order.

%Alternatively the attitude can obtained computing a Jacobi elliptic integral of the third kind \cite{celledoni08tuo}.

Once $\mbox{\boldmath $\omega$}$ and $Q$ are computed to the desired accuracy, $\mathbf{p}$ can be easily obtained by
$$
\begin{array}{rcl}
\mathbf{p}(\gamma) &=& Q^TQ_0\mathbf{p}_0, \\
%\dot{\mathbf{x}} &=& Q\mathbf{v} = Q Q^TQ_0 \mathbf{v}_0 = Q_0\mathbf{v}_0,
\end{array}
$$
while
\begin{eqnarray*}
\mbox{\boldmath $\mu$}(\gamma)&=& \mbox{\boldmath $\mu$}_0,\\
\mathbf{x}(\gamma)&=&\mathbf{x}_0,\\
\mbox{\boldmath $\varphi$}_q(\gamma)&=& \mbox{\boldmath $\varphi$}_{q,0},\\ 
\mbox{\boldmath $\varphi$}_x(\gamma)&=&\mbox{\boldmath $\varphi$}_{x,0}.
\end{eqnarray*}
%$$\mbox{\boldmath $\mu$}(\gamma)= \mbox{\boldmath $\mu$}_0,$$
%$$\mathbf{x}(\gamma)=\mathbf{x}_0.$$
%$$\mathbf{x}(\gamma)=\mathbf{x}_0+\gamma \, Q_0\mathbf{v}_0.$$

%\noindent where $\mathbbm{q}$ is the Euler parameter describing the rotation of the
%body and $\Omega = \left(0,T^{-1}\mathbf{m}\right) =
%\left(0,\mbox{\boldmath $\omega$} \right)$.

%Finally we obtain
%\begin{eqnarray*}
%%\mbox{\boldmath $\varphi$}_q(\gamma)&=& \mbox{\boldmath $\varphi$}_{q,0},\\ % \int_{0}^{\alpha(h)}\mbox{\boldmath $\theta$}(Q(s))\,\,ds-\alpha(h)\mbox{\boldmath $\theta$}_0,\\
%\mbox{\boldmath $\varphi$}_x(\gamma)&=&\mbox{\boldmath $\varphi$}_{x,0}+\gamma\,\tilde{\mathbf{x}}_0. \\%+\frac{1}{2}\gamma^2Q_0\mathbf{v}_0, \quad \gamma\in [0,\alpha h].\\
%%(\mbox{\boldmath $\varphi$}_x(\gamma)&=&\mbox{\boldmath $\varphi$}_{x,0}+\gamma\tilde{\mathbf{x}}_0+\frac{1}{2}\gamma^2Q_0\mathbf{v}_0, \quad \gamma\in [0,\alpha h].)\\
%\end{eqnarray*}
The rotational part of the equations evolves on $SO(3)$. The Magnus method respects the manifold structure of this Lie gorup. Compared to using Euler angles, this approach avoids singularities by construction. 
This may not be important when simulating the vessel alone, because only a certain limited range of rotations are allowed. However, it becomes more difficult to avoid the singularities of Euler angles  when considering the attitude of the vessel and of each cross sections of the pipe simultaneously,  \cite{jensen10anp}.
The Magnus expansion (which by construction provides an attitude that evolves on $SO(3)$) can also be applied when the mass matrix of the system is more general and the added mass matrix is not diagonal.

\subsubsection{System $\mathbf{S_2}$: Integration of the damping, gravitational and control forces.}

It is easy to realize that the system of differential equations $\mathbf{S_2}$ % free rigid body equations
\begin{equation}
\label{eq:vflows2}
\mathbf{S_2} = \left\{\begin{aligned}
\dot{\mathbf{p}} &=  -\left(D_tm_v^{-1}\mathbf{p}+Q^T\mathcal{A}\mathbf{x}-\mbox{\boldmath $\tau$}_t\right),\\
\dot{\mathbf{m}} &= - \left(D_rT^{-1}\mathbf{m}+\widehat{\mbox{\boldmath $\mu$}}\,\mathbf{q}_3-\mbox{\boldmath $\tau$}_r\right),\\
%A^{(2)}\mathbf{m}
%+ \mathbf{w}_1^{(2)} + \mathbf{w}_2^{(2)} t,\\
%\left( A^{(1)}\mathbf{v} + \mathbf{w}_1^{(1)}
%+ \mathbf{w}_2^{(1)}t   \right),\\
\dot{Q}&= \mathbf{0},\\
\dot{\mbox{\boldmath $\mu$}}&= - \mathcal{G}\,\widehat{\mbox{\boldmath $\omega$}}\, \mathbf{q}_3,\\
\dot{\mathbf{x}} &= Q\mathbf{v}, \\
\dot{\mbox{\boldmath $\varphi$}}_{\boldsymbol{\theta}}&=\tilde{\mbox{\boldmath $\theta$}}, \\
\dot{\mbox{\boldmath $\varphi$}}_{\mathbf{x}}&=\tilde{\mathbf{x}}.%\mathbf{0}
\end{aligned} \right. 
\end{equation}
is linear. As with the system $\mathbf{S_1}$, $\mathbf{S_2}$ should be integrated several times on some interval $[0,\beta h]$, where $\beta$ is $b_1,\, b_2,\dots,b_{m}$, i.e. one of the coefficients of the splitting method. Using \eqref{controls1}, \eqref{controls2}, \eqref{controls3} and the variation of constants formula we obtain the following explicit expressions for the solution of \eqref{eq:vflows2}
\begin{align*}
Q(\gamma) &= Q_0,\\
\mbox{\boldmath $\varphi$}_{\boldsymbol{\theta}}(\gamma)&=\mbox{\boldmath $\varphi$}_{\boldsymbol{\theta},0}+\gamma\, \tilde{\mbox{\boldmath $\theta$}}_0, \hskip0.5cm \tilde{\mbox{\boldmath $\theta$}}_0:=\mbox{\boldmath $\theta$}_0-\mbox{\boldmath $\theta$}_{ref}, \\[0.2cm]
%\mbox{\boldmath $\varphi$}_{\mathbf{x}}(\gamma)&=\mbox{\boldmath $\varphi$}_{\mathbf{x},0},\\
\left[\begin{array}{c}
\mathbf{m}(\gamma)\\
\mbox{\boldmath $\mu$}(\gamma)
\end{array}\right]&=e^{\gamma A}\, \left[\begin{array}{c}
\mathbf{m}_0\\
\mbox{\boldmath $\mu$}_0
\end{array}\right] +\gamma \,\phi_1(\gamma A)\left[\begin{array}{c}
\mathbf{w}_{r,1}\\
\mathbf{0}
\end{array}\right]+\gamma^2\,\phi_2(\gamma A)\left[\begin{array}{c}
\mathbf{w}_{r,2}\\
\mathbf{0}
\end{array}\right],\\
%\mbox{\boldmath $\omega$} (\gamma) &=  e^{\gamma A} \mbox{\boldmath $\omega$}_0+ \gamma \,\phi_1(\gamma A)\mathbf{w}_{r,1},+\gamma^2\,\phi_2(\gamma A)\mathbf{w}_{r,2},\\
%-D_RT^{-1}\mathbf{m}-Q^T\mathbf{g}_r^s+\mbox{\boldmath $\tau$}_2\\
%A^{(2)}\mathbf{m}
%+ \mathbf{w}_1^{(2)} + \mathbf{w}_2^{(2)} t,\\
\left[\begin{array}{c}
\mathbf{p}(\gamma)\\
\mathbf{x}(\gamma)\\
\mbox{\boldmath $\varphi$}_{\mathbf{x}}(\gamma)
\end{array}\right]&=e^{\gamma B}\, \left[\begin{array}{c}
\mathbf{p}_0\\
\mathbf{x}_0\\
\mbox{\boldmath $\varphi$}_{\mathbf{x},0}
\end{array}\right] +\gamma \,\phi_1(\gamma B)\left[\begin{array}{c}
\mathbf{w}_t\\
\mathbf{0}\\
-\mathbf{x}_{ref}
\end{array}\right],\\
%\mathbf{v}(\gamma) &=  e^{\gamma B}\mathbf{v}_0+\gamma\,\phi_1(\gamma B) \mathbf{w}_t, \\%m_v^{-1}\left(D_T\mathbf{v}+Q^T\mathbf{g}_t^s-\mbox{\boldmath $\tau$}_1\right)\\
%\left( A^{(1)}\mathbf{v} + \mathbf{w}_1^{(1)}
%+ \mathbf{w}_2^{(1)}t   \right),\\
%\mathbf{x} (\gamma)&= \mathbf{x}_0, 
\end{align*}
where
{\scriptsize
$$A:=\left[\begin{array}{cc}
-(D_rT^{-1}+Q_0^T\Pi_e^{-T}K_d^r\Pi_e^{-1}Q_0T^{-1}) & \widehat{q_3}\\[0.3cm]
\mathcal{G}\widehat{q_3}T^{-1} & O\\
\end{array}\right]
,
$$
$$
B:=
\left[\begin{array}{ccc}
-(D_tm_v^{-1}+Q_0^TK_d^tQ_0m_v^{-1}), & -(Q_0^T\mathcal{A}+Q_0^TK_p^t) & -Q_0^TK_i^t \\[0.3cm]
Q_0m_v^{-1} & O & O\\[0.2cm]
O & I  & O
\end{array}\right],$$
}
\begin{align*}
\mathbf{w}_{r,1}& :=-Q_0^T\Pi_e^{-T}(K_p^r \tilde{\mbox{\boldmath $\theta$}}_0+K_i^r\mbox{\boldmath $\varphi$}_{\boldsymbol{\theta},0}),\\
\mathbf{w}_{r,2}& :=-Q_0^T\Pi_e^{-T}K_i^r\tilde{\mbox{\boldmath $\theta$}}_0, \\
%\mathbf{w}_t& = -m_v^{-1}Q_0^T(K_p^t\tilde{\mathbf{x}}_0+K_i^t\,\mbox{\boldmath $\varphi$}_{\mathbf{x},0}),\\
\mathbf{w}_t& := Q_0^T(K_p^t\,\mathbf{x}_{ref}),
\end{align*}
and 
$$\phi_k(z) = \frac{1}{(k - 1)!} \int_0^1 e^{z (1-x)} x^{k-1} \,dx, \quad k=1,2.$$ %\frac{e^z-1}{z},\quad \phi_2(z)=
From the variation of constants formula we deduce
{\small
$$\gamma \,\phi_1(\gamma A)\left[\begin{array}{c}
\mathbf{w}_{r,1}\\
\mathbf{0}
\end{array}\right]+\gamma^2\,\phi_2(\gamma A)\left[\begin{array}{c}
\mathbf{w}_{r,2}\\
\mathbf{0}
\end{array}\right]=-\int_0^{\gamma}e^{(\gamma-\sigma)A}Q_0^T\Pi_e^{-T}(K_p^{r}\tilde{\mbox{\boldmath $\theta$}}
 + K_i^{r} \mbox{\boldmath $\varphi$}_{\boldsymbol{\theta}}(\sigma))\, d\sigma,$$
 }
 where $\tilde{\mbox{\boldmath $\theta$}}$ does not depend on $\sigma$.


==> Submission arXiv/Chapters/5_Numerical_results.tex <==
\section{Numerical results}
\label{experiments}




In this section we report the results of some numerical experiments for %
\eqref{eq:vessel}. The parameter values used for the rigid body vessel model are given in Appendix \ref{ParamValues}. For the parametrization of the rotation matrices we have used unit quaternions, see  Appendix \ref{quatEq}. The reference solution has been computed with the classical Runge-Kutta method of order $4$ (RK4) with small step size $h = 10^{-6}$ in the order tests, Figure~\ref{order}, and $h = 10^{-4}$ in the other experiments. %, 

In Figure \ref{evo}, we show the features of the solution of the considered controlled system, and see that the desired equilibrium is attained. We plot the evolution of the generalized positional coordinates over the interval $t \in [0,200]$. The controls are turned on at $t=50$, \cite{jensen09mac}. Let us denote by $x$ and $y$ the first two components of the vector $\mathbf{x}$, and recall that $\psi$ is the third component of $\boldsymbol{\theta}$. The results show rapid convergence towards the reference values for $x$, $y$ and $\psi$. There is a slight initial overshoot due to the presence of the integral term, which will vanish over time. The overshoot can be reduced by 
further optimizing the choice of controller gains. In our experiments, choosing different values for the environmental forces, we observe that the integral term is in general necessary to ensure convergence to the set point, see also \cite{jensen09mac}. The uncontrolled variables show expected behaviour. The remaining angles have small initial oscillations which are damped towards 0. In the case of $\phi$ the damping is present, but too small to be observed from the plot. When the controls are turned on, the elevation $z$ moves away from the equilibrium, but it rapidly stabilises back to the desired value.

\begin{figure}
  \centering 
   \includegraphics[width=1\textwidth]{Figures/Evolution}
\caption{Evolution of the generalized position variables over time with $t \in [0,200]$. The PID controller is turned on at $t=50$. All the controlled variables converge rapidly towards the reference values, with a small overshoot caused by the integral term in the controller.  \label{evo}}
  
\end{figure}


We now verify the order of accuracy of the numerical solutions obtained by the order 2, order 4 and order 6 splitting schemes, which we will refer to as SP2, SP4 and SP6, respectively. We define the relative error for the angular momentum at time $t_n$
$$
e^{[\mathbf{m}]} = \frac{\vectornorm{\mathbf{m}_n-\mathbf{m}(t_n)}_2}{\vectornorm{\mathbf{m}(t_n)}_2},
$$
where $\mathbf{m}(t_n)$
is the reference solution, and $\mathbf{m}_n \approx \mathbf{m}(t_n)$ is the approximation given by the numerical method whose accuracy we want to investigate. Similar relative errors $e^{[q]}$, $e^{[\mathbf{v}]} $ and $e^{[\mathbf{x}]} $ are considered for $q$, $\mathbf{v}$ and $\mathbf{x}$, respectively. Here $q$ is the unit quaternion representing the attitude $Q$. The errors are evaluated at the end of the time interval, $t\in [0,1]$. In Figure \ref{order} we plot the relative errors against the step size for step sizes $h_{k} =\frac{1}{2^k}$  with $k =0,1,\hdots,4$, and show that the correct order is attained by the methods.

%?????
%
%We now verify the order of accuracy of the numerical solutions obtained by the order 2 and order 4 %and order 6 
%splitting schemes, which we will refer to as SP2, SP4 %and SP6 
%respectively. We denote with $\mathbf{y} := [
%\mathbf{p}^T, \mathbf{m}^T, q, \mbox{\boldmath $\mu$}^T, \mathbf{x}^T ,\mbox{\boldmath $\varphi$}_{\boldsymbol{\theta}}^T, \mbox{\boldmath $\varphi$}_{\mathbf{x}}^T]$, where $q$ is the unit quaternion representing the attitude rotation $Q$.
%We define the relative error at time $t_n$
%%$$
%%e^{[\mbox{\boldmath $\omega$}]} = \frac{\vectornorm{\mbox{\boldmath $\omega$}_n-\mbox{\boldmath $\omega$}(t_n)}_2}{\vectornorm{\mbox{\boldmath $\omega$}(t_n)}_2},
%%$$
%$$
%e^{[\mathbf{y}]} = \frac{\vectornorm{\mathbf{y}_n-\mathbf{y}(t_n)}_2}{\vectornorm{\mathbf{y}(t_n)}_2},
%$$
%where $\mathbf{y}(t_n)$
%is the reference solution, and $\mathbf{y}_n \approx \mathbf{y}(t_n)$ is the approximation given by the numerical method whose accuracy we want to investigate. %Similar relative errors $e^{[\boldsymbol{\theta}]}$, $e^{[\mathbf{v}]} $ and $e^{[\mathbf{x}]} $ are considered for $\boldsymbol{\theta}$, $\mathbf{v}$ and $\mathbf{x}$, respectively. 
%The errors are evaluated at the end of the time interval, $t\in [0,10]$. In Figure \ref{order} we plot the relative errors against the step size for step sizes $h_{k} =\frac{1}{2^k}$  with $k =0,1,\hdots, 5$ and show that the correct order is attained for the methods.

\begin{figure}
  \includegraphics[width=0.85\textwidth]{Figures/Ordertest27Mar}%Converg}
\caption{Dependence of the relative endpoint error ($y$-axis) on the size of the integration step ($x$-axis) for \eqref{eq:vflows}. 
%various solution components. From top left angular velocity $\mbox{\boldmath $\omega$}$, orientation $\mbox{\boldmath $\theta$}$, velocity $\mathbf{v}$ and position $\mathbf{x}$.  
Results for SP2, SP4 
and SP6 
are plotted in logarithmic scale for $t \in [0,1]$, $h=\frac{1}{2^k}$ and $k=0,1,\hdots , 4$. Top: global error in angular momentum $\mathbf{m}$ (left) and attitude $q$ (right). Bottom: global error in linear momentum $\mathbf{p}$ and position $\mathbf{x}$. The expected order for the splitting schemes is obtained. \label{order}}
\end{figure}

Finally, in Figure \ref{EnErrorEvo}, we compare the norm of the scaled control input and the energy  function $H$, given by  \eqref{Hamiltonian} for the splitting methods SP2 and SP4, and two explicit Runge-Kutta methods: the Improved Euler method (a second order Runge-Kutta method\footnote{$y_{n+1}=y_n+\frac{h}{2}\big( f(y_n)+f(y_n+hf(y_n))\big)$}) and RK4. Methods of the same order are compared using relatively large step sizes, specifically $h=2/3$ (top figures) and $h=1.9375$ (bottom figures). The values from the splitting methods in this experiment cannot be distinguished from the corresponding values from the exact solution, while the values from the explicit Runge-Kutta methods differ noticeably. For larger values of the step-sizes the explicit Runge-Kutta methods are unstable. A more detailed analysis of the stability and of the error of splitting methods for similar problems in rigid body dynamics is under investigation. Preliminary results show that as $h$ increases, splitting methods suffer of order reduction, but they do not become unstable and the error remains bounded. This is similar to what shown in the case of Schr{\"o}dinger equations, see \cite{janke}. %, in particular for the rotational part.

%\begin{figure}
%  \includegraphics[width=1\textwidth]{Figures/torque_trans_rot}
%\caption{The norm of the scaled rotational control $\left\|T^{-1}\boldsymbol{\tau}_r\right\|_2$ (left) and scaled translational control $\left\|m_v^{-1}\boldsymbol{\tau}_t\right\|_2$ (right) for time $t \in [0,110]$ are shown. In both plots the values from the splitting method and the RK4 method, both 4th order, with step size $h = 1.95$, are compared against the exact solution. The values from the splitting method are seen to be virtually indistinguishable from the exact solution. On the contrary, the values from RK4 are seen to differ, especially for the rotational part. \label{torque}}
%\end{figure}

%In Table \ref{enComp} we compare the relative energy errors for different methods at the endpoint of a long time simulation, $t \in [0,50 000]$, for a range of different step sizes. The reference solution is here computed using RK4 with $h = 0.005$. SP2 and SP4 are compared to two explicit Runge-Kutta methods of the same order, namely improved Euler and RK4 respectively. The table also illustrates the stability of the methods. In both the 2nd and 4th order case the splitting methods are seen to be stable for significantly larger step sizes. The energy at the endpoint is well approximated even close to their step size limit. Improved Euler becomes unstable even for fairly small step sizes, with a long term energy which increases exponentially. RK4 has significant artificial damping for larger step sizes, leading to an energy which is damped too fast towards 0 and an error that approaches 1, before the method becomes unstable.
%
%
%The aforementioned artificial damping of RK4 is easily observed in Figure \ref{EnErrorEvo}. Here we plot the evolution of the approximate scaled energy $H_n/H_0$ for RK4 and SP4 using $h = 1.95$. We also include SP4 with $h = 5$ to show that even close to instability, the splitting method gives a qualitatively correct evolution of the energy.

\begin{figure}
  \centering 
     \includegraphics[width=1\textwidth]{Figures/energyO2O4}
\caption{Time versus the scaled energy $H(y_n)/H_0$ (left) and time versus the norm of the scaled rotational control $\left\|T^{-1}\boldsymbol{\tau}_r\right\|_2$ (right). The two top figures compare the methods of order 2: SP2 and Improved Euler, for time $t \in [0,50]$ and step size $h=2/3$. The two bottom figures compare methods of order $4$: SP4 and RK4 with step size $h = 1.9375$ on the time interval $[0,100]$. All methods are compared with the exact solution. The splitting methods follow the exact scaled energy and torque well. On the contrary, the values from the RK4 and of the Improved Euler method are seen to differ.  \label{EnErrorEvo}}
\end{figure}

%In Table \ref{GEcomp} we compare the relative global errors for the same methods at the endpoint of a simulation, $t \in [0,780]$. Note first that RK4 is close to its convergence limit for $h=0.005$, which serves to justify the use of RK4 with $h=0.005$ as the exact solution for the longer simulation. All methods are seen to have the expected order. Similarly to the results in Table \ref{enComp}, the splitting methods give lower errors, and are stable for larger step sizes than the comparison RK-method of the same order. 





==> Submission arXiv/Chapters/6_Concluding_remarks.tex <==
\section{Concluding remarks}
\label{conclusion}
We have proposed a class of splitting schemes for a system of controlled vessel rigid body equations in use in offshore marine operations. %The vessel equations are input-output passive and the methods preserve this property under numerical time-discretization. %are specifically tailored for this problem, i.e. for a rigid body problem including rotational and translational motion in presence of external forces, damping and controls.  %Something about these equations not being trivial to formulate.
The discrete systems respect important qualitative features of the continuous system: we have proved that the numerical flow obtained by the splitting methods is input-output passive, and the numerical attitude  evolves on the Lie group $SO(3)$ as its continuous counterpart.
The benefit of the passivity-preserving schemes is that they satisfy a definition of passivity analogous to the one satisfied by the continuous equations. The control of the continuous system is designed so to guarantee the attainment of a certain desired equilibrium, but ultimately the systems are discretized with numerical integration techniques. The passivity preserving schemes ensure this same property at the discrete level by construction of the numerical methods.

With the proposed splitting schemes we achieve improved accuracy in the numerical solution. In our numerical experiments the methods show better energy behaviour compared to classical Runge-Kutta techniques. 




The splitting methods considered have not been optimised with respect to global error, number of stages, i.e. elementary flows composed, and computational effort. %A proper study of passivity preserving splitting methods of order higher than $2$ using complex coefficients with positive real part \cite{blanesComplexcoeff} will be subject of future investigations. 
This is future work. A reformulation of the input forces using only the attitude  and the angular velocity, and a general improvement of the controlled system will  also be considered in the future. 
%Something about passivity. %The splitting schemes create a powerful platform for improving existing numerical integration methods with respect to passivity/energy preservation.

==> Submission arXiv/Chapters/Bibliography.tex <==
%%%%%%%%%%%%%%%%%%%
%  BIBLIOGRAPHY:  %
%%%%%%%%%%%%%%%%%%%
\begin{thebibliography}{9}

\bibitem{baker02mg}
Baker A.
\newblock {\em Matrix Groups: An Introduction to Lie Group Theory. Springer Undergraduate Mathematics Series}. 
\newblock Springer-Verlag: London, 2002.
\newblock 

\bibitem{blanes}
Blanes S, Casas F, Murua A.
\newblock{Splitting methods in the numerical integration of non-autonomous dynamical systems}.
\newblock{\em Revista de la Real Academia de Ciencias Exactas, Fisicas y Naturales. Serie A. Matematicas} 2012; \textbf{106}(1):49--66. DOI: 10.1007/s13398-011-0024-8.

\bibitem{blanesComplexcoeff}
Blanes S, Casas F, Murua A.
\newblock{Splitting methods with complex coefficients}
\newblock{\em Bol. Soc. Esp. Mat. Apl.} 50(2010), 47--61.


\bibitem{blanes02}
Blanes S, Casas F, Ros J.
\newblock{High order optimised geometric integrators for linear differential equations}.
\newblock{\em BIT Numerical Mathematics} 2002; \textbf{42}(2): 262--284. DOI: 10.1023/A:1021942823832.


\bibitem{BM} N. Bou Rabee and J. E.  Marsden, \textit{Hamilton-Pontryagin Integrators on Lie Groups Part I: Introduction and Structure-Preserving Properties}, Found Comput Math (2009) 9: 197--219. DOI 10.1007/s10208-008-9030-4.

\bibitem{celledoni09epr}
E. Celledoni, R.I. McLachlan, D.I. McLaren, B. Owren, G.W.R. Quispel and W. Wright, 
\newblock\textit{Energy-preserving Runge-Kutta methods}. 
\newblock{M2AN (Mathematical Modelling and Numerical Analysis)}, vol 43 (4), 645-649, (2009). 

\bibitem{celledoni06ets}
Celledoni E, S{\"a}fstr{\"o}m N.
\newblock{Efficient time-symmetric simulation of torqued rigid bodies using Jacobi elliptic functions}.
\newblock{\em Journal of Physics A} 2006; \textbf{39}(19):5463--5478. DOI: 10.1088/0305-4470/39/19/S08.

\bibitem{celledoni08tec}
Celledoni E, Fass{\`o} F, S{\"a}fstr{\"o}m N, Zanna A.
\newblock{ The exact computation of the free rigid body motion and its use in splitting methods}.
\newblock{\em SIAM Journal on Scientific Computing} 2008; \textbf{30}(4):2084--2112. DOI: 10.1137/070704393.

\bibitem{celledoni10frb}
Celledoni E, Zanna A.
\newblock{ Algorithm 903: FRB-Fortran routines for the exact computation of free rigid body motions}.
\newblock{\em ACM Transactions on Mathematical Software} 2010; \textbf{37}(2):23:1--23:24. DOI: 10.1145/1731022.1731033.

\bibitem{egeland}
Egeland O, Gravdahl JT.
\newblock{\em Modeling and Simulation for Automatic Control}. Corrected second printing 2003. 
\newblock Marine Cybernetics: Trondheim, 2002.




\bibitem{marinecontrolsystems}
Fossen TI.
\newblock{\em Marine Control Systems}.
\newblock  Marine Cybernetics: Trondheim, 2002.


\bibitem{jensen09mac}
  {Jensen GA, S{\"a}fstr{\"o}m N, Nguyen TD, Fossen TI}.
\newblock{Modeling and control of offshore pipelay operations based on a finite strain pipe model}.
\newblock{\em Proceedings of American Control Conference}, St. Louis, MO, USA, 2009; 4717--4722. DOI: 10.1109/ACC.2009.5160110.

\bibitem{jensen10anp}
Jensen GA, S{\"a}fstr{\"o}m N, Nguyen TD, Fossen TI.
\newblock{A nonlinear PDE formulation for offshore vessel pipeline installation}.
\newblock{\em Ocean Engineering} 2010; \textbf{37}(4):365--377. DOI: 10.1016/j.oceaneng.2009.12.009.


\bibitem{gustavson}
Gustafsson E.
\newblock{Accurate discretizations of torqued rigid body dynamics}.
\newblock{\em Master thesis, Norwegian University of Science and Technology}: Trondheim, 2010.

\bibitem{hairer}
E. Hairer
\newblock{\em Energy-preserving variant of collocation methods}
\newblock{Journal of Numerical Analysis, Industrial and Applied Mathematics} 5, 73-84, (2010).

\bibitem{gni06hairer}
E. Hairer, C. Lubich and G. Wanner
\newblock{\em Geometric Numerical Integration} 
\newblock Springer series in Computational Mathematics, {\bf 31}, Springer (2006).


\bibitem{hairer91sod}
E. Hairer and G. Wanner
\newblock{\em Solving odrinary differential equations II} 
\newblock Springer series in Computational Mathematics, {\bf 14}, Springer.



\bibitem{holm}
Holm Darryl D,
\newblock{\em Geometric Mechanics, Part II:
Rotating, Translating and Rolling} 
\newblock Mathematics Department
Imperial College London.

\bibitem{lamb}
H. Lamb, 
\newblock{\em Hydrodynamics}, 
\newblock Cambridge University press, fourth edition, 1916.


\bibitem{Kirchhoff}
Kirchhoff G. R., 
\newblock{\em Ueber die Bewegung eines Rotationsk{\"o}rpers i einer Fl{\"u}ssigkeit}, 
\newblock Crelle t. lxxi, (1869) [Ges. Abh. p.376], Mechanik, c. xix.

\bibitem{marsden99IMS}
Marsden JE, Ratiu TS.
\newblock {\em Introduction to Mechanics and Symmetry: A Basic Exposition of Classical Mechanical Systems.} Second edition. Vol. 17 of {\em Texts in Applied Mathematics}.  
\newblock Springer-Verlag: New York, 1999.

\bibitem{marsdenwest}
Marsden JE, and West M.
\newblock {\em Discrete mechanics and variational integrators}, 
\newblock Acta Numerica, 10 (2001), pp. 357--514.

\bibitem{mclachlanDG}
McLachlan RI, Quispel GRW, Robidoux N
\newblock{\em Geometric integration using discrete gradients}
\newblock{ Philosophical Transactions of the Royal Society of London A: Mathematical, Physical and Engineering Sciences} 357, 1021--1045.

\bibitem{mss}
\newblock{\em MSS. Marine Systems Simulator}, 2010. 
\newblock Viewed 2014-04-04, http://www.marinecontrol.org.

\bibitem{muller}
A. M{\"u}ller,
\newblock{\em Screw and Lie group theory in rigid body dynamics},
\newblock{Multibody Syst. Dyn.} (2018) 42:219--248,
DOI 10.1007/s11044-017-9583-6

\bibitem{janke}
T. Jahnke and C. Lubich
\newblock{\em Error bounds for exponential operator splitting},
\newblock{BIT Num. Math.}, 40, 735--744, (2000).


\bibitem{perez07kmf}
Perez T, Fossen TI.
\newblock {Kinematic models for manoeuvring and seakeeping of marine vessels}.
\newblock{\em Modeling, Identification and Control} 2007; \textbf{28}(1):19--30. DOI: 10.4173/mic.2007.1.3.


\bibitem{safstrom09mas}
S{\"a}fstr{\"o}m N. 
\newblock{Modeling and simulation of rigid body and rod dynamics
  via geometric methods}.
\newblock{\em PhD thesis, Norwegian University of Science and Technology}: Trondheim, 2009.


\bibitem{VanderSchaft06pHs}
Van der Schaft A. 
\newblock{Port-{H}amiltonian systems: an introductory survey}.
\newblock{\em European Mathematical Society Publishing House (EMS Ph)}: 2006.


\end{thebibliography}

%**********************************************************************************************************



%\bibitem{blanes09tme}
%S. Blanes, F. Casas, J.A. Oteo and J. Ros.
%\newblock The Magnus expansions and some of its applications. 
%\newblock{\em Phys. Rep.}, 470(5-6):151-238, 2009.

%\bibitem{blanes02tme}
%S. Blanes, P.C. Moan.
%\newblock{\em Practical Symplectic Partitioned Runge-Kutta and Runge-Kutta-Nystr{\"o}m Methods}.
%\newblock JCAM, 142(2):313-330, 2002.

%\bibitem{fossen04ntd}
% T.I. ~Fossen and {\O}.N.~Smogeli.
%\newblock{\em Nonlinear Time-Domain Strip Theory Formulation for Low-Speed Maneuvering and Station-Keeping}.
%\newblock Modelling, Identification and Control, MIC-25(4):201--221, 2004.

%\bibitem{hairer06gni}
%E.~Hairer, C.~Lubich, and G.~Wanner.
%\newblock{\em Geometric Numerical Integration}, volume~31 of {\em Springer
%  Series in Computational Mathematics}.
%\newblock Springer-Verlag, Berlin, second edition, 2006.
%\newblock Structure-Preserving Algorithms for Ordinary Differential Equations.  

%\bibitem{leimkuhler04shd}
%B.~Leimkuhler, S.~Reich.
%\newblock{\em Simulating Hamiltonian Dynamics}, Vol.~14 of {\em Cambridge Monographs on Applied and Computational
%  Mathematics}.
%\newblock Cambridge University Press, first edition, 2004.

%\bibitem{maciejewski85hfep}
%A.~J. Maciejewski.
%\newblock{\em Hamiltonian formalism for Euler parameters}.
%\newblock Celestial Mech., 37:47--57, 1985.

%\bibitem{mclachlan02sm}
%R.~I. McLachlan and G.~R.~W. Quispel.
%\newblock{\em Splitting Methods}.
%\newblock Acta Numer., 11:341--434, 2002. 

%\bibitem{whittaker37ato}
%E.~T. Whittaker.
%\newblock {\em A Treatise on the Analytical Dynamics of Particles and Rigid
%  Bodies}
%\newblock Cambridge University Press, fourth edition, 1937.

%\bibitem{yoshida90coh}
%H.~Yoshida.
%\newblock{\em Construction of Higher Order Symplectic Integrators}.
%\newblock Physics Letters A, 150:262--268, 1990.





==> Submission arXiv/Chapters/Section2.tex <==
\section{Energy conservation and passivity } % a.k.a. Passivity
\label{passivity}

In the present section we consider the problem of conservation of the total energy. 
%Starting from the formal definition of the law of energy conservation for isolated (closed-loop) systems, one can write the Hamiltonian $H = H(t)$ at a %given time $t$ as
%\begin{equation}
%H = H_0 + A_{ext} %\Big|_0^t
%\label{eq:total_energy}
%\end{equation}
%~\ref{eq:total_energy}
%where $A_{ext}$ is the work of external forces on the vessel.
In terms of control dynamics, the systems of interest are frequently considered as nearly isolated, and the energy conservation law is formulated in terms of the \textit{passivity} of the system.  We will use %will show that our system satisfies 
the following definition of passivity.
\begin{defn}
\label{defpass} \cite{egeland} (Chapter 2)
\newline
Consider a model 
\begin{align*}
\dot {\mathbf{y}}  &= \mathbf{f}(\mathbf{y}, \, \mathbf{u}), \\
\boldsymbol{\zeta} &=\mathbf{h}(\mathbf{y}).
\end{align*}
Suppose that there is a \emph{storage function} $V(\mathbf{y})\geq 0$ and a dissipation function $g(\mathbf{y}) \geq 0$ so that the time derivative of $V$ for a solution of the system satisfies 
\begin{equation*}
\dot{V}=\nabla V(\mathbf{y})^T\mathbf{f}(\mathbf{y}, \, \mathbf{u})= \mathbf{u}^T \boldsymbol{\zeta}-g(\mathbf{y}),
\end{equation*} 
 for all control inputs $\mathbf{u}$. Then the system with input $\mathbf{u}$ and output $\boldsymbol{\zeta}$ is said to be (input-output) passive. 
\end{defn}

Notice that the passivity condition is equivalent to
\begin{equation}
\label{passivity1}
V(\mathbf{y}(t))-V(\mathbf{y}(0))=\int_0^t\left(\mathbf{u}(s)^T \boldsymbol{\zeta}(s)-g(\mathbf{y}(s))\right)\,ds.
\end{equation}

Let $H:\mathbf{R}^m\rightarrow\mathbf{R}$ be a total energy function, $\mbox{\boldmath $\xi$}(t)\in\mathbf{R}^m$, $\mbox{\boldmath $\tau$}(t)\in\mathbf{R}^p$, $S(\mbox{\boldmath $\xi$})\in \mathbf{R}^{m\times m}$ skew-symmetric,  $G(\mbox{\boldmath $\xi$})\in \mathbf{R}^{m\times p}$, $D(\mbox{\boldmath $\xi$})\in \mathbf{R}^{p\times p}$ positive definite.
Consider the system 
%The system \eqref{eq:vessel} can be written in the form
\begin{eqnarray}
\label{eq:xiDiff}
\dot{\mbox{\boldmath $\xi$}} &=& S(\mbox{\boldmath $\xi$})\nabla H(\mbox{\boldmath $\xi$}) -G\left(D(\mbox{\boldmath $\xi$})\mbox{\boldmath $\nu$} - \mbox{\boldmath $\tau$}\right),\\
\mbox{\boldmath $\nu$}&=&G^T\nabla H(\mbox{\boldmath $\xi$})
\end{eqnarray}
also known as an input-state-output port-Hamiltonian system with input $\mbox{\boldmath $\tau$}$ and output $\mbox{\boldmath $\nu$}$, \cite{VanderSchaft06pHs}.
%with %$\mbox{\boldmath $\nu$}:=G^T\nabla H(\mbox{\boldmath $\xi$})$, 
%$D(\mbox{\boldmath $\xi$})$ positive definite and $S(\mbox{\boldmath $\xi$})$ skew-symmetric
%\eqref{eq:xiDiff} 
\begin{Proposition}\label{passivityPROP} The system \eqref{eq:xiDiff}  
is input-output passive with input $\mbox{\boldmath $\tau$}$ and output $\mbox{\boldmath $\nu$}$.
\end{Proposition}

\begin{proof}
Differentiating $H$ with respect to time and using \eqref{eq:xiDiff} we find
\begin{equation}
\dot{H} = \nabla H(\mbox{\boldmath $\xi$})^T\dot{\mbox{\boldmath $\xi$}} = \nabla H(\mbox{\boldmath $\xi$})^T S(\mbox{\boldmath $\xi$})\nabla H(\mbox{\boldmath $\xi$}) +  \mbox{\boldmath $\nu$}^T (-D \mbox{\boldmath $\nu$} + \mbox{\boldmath $\tau$}) = \mbox{\boldmath $\nu$}^T (-D \mbox{\boldmath $\nu$} + \mbox{\boldmath $\tau$}),
\label{eq:HamDiff}
\end{equation}
where the last equality in \eqref{eq:HamDiff} follows from the skew symmetry of $S$.

If we choose $V = H$, $\mathbf{y} = \mbox{\boldmath $\xi$}$, $\mathbf{u}=\mbox{\boldmath $\tau$}$ and $\boldsymbol{\zeta}=\mbox{\boldmath $\nu$}$, then it follows from \eqref{eq:HamDiff} that the system \eqref{eq:xiDiff} satisfies Definition \ref{defpass} with  $g(\mathbf{y})=\mbox{\boldmath $\nu$}^T \, D \mbox{\boldmath $\nu$}$ and $\mathbf{h}(\mathbf{y}) =G^T\nabla H(\mbox{\boldmath $\xi$})$. Thus the system is passive. The requirement $g(\mathbf{y}) \geq 0$ is fulfilled because the matrix $D$ is positive-definite. 
\end{proof}

%\section{Passivity and interconnection for the vessel equations}

%For the vessel model, we now define $\mbox{\boldmath $\xi$} := [
%\mathbf{p}^T, \mathbf{m}^T, \mathbf{q}_1^T, \mathbf{q}_2^T, \mathbf{q}_3^T, \mbox{\boldmath $\mu$}^T, \mathbf{x}^T ]$
%with
%$$
%\mathbf{p} := m_v \mathbf{v}, \quad\mathbf{m} := T\boldsymbol{\omega},  \quad \mathbf{q}_i := Q^T\mathbf{e_i},\quad \mbox{\boldmath $\mu$}:=\mathcal{G}\mathbf{q}_3,
%$$
%with $m_v$ and $T$ diagonal and invertible matrices.
%Taking $H = H(\mbox{\boldmath $\xi$})$ to be the Hamiltonian of the system, given as the sum of the kinetic energy $K$ and the potential energy $U$, 
%assuming
%$$\mathcal{A}  := \mathrm{diag}(0,0,c), \quad \mathcal{G}  := m_v g\, \mathrm{diag}(\overline{GM}_L,\overline{GM}_T,0),\quad \tilde{\mathcal{G} } := \frac{1}{m_v g}\, \mathrm{diag}((\overline{GM}_L)^{-1},(\overline{GM}_T)^{-1},0),$$
%and $c := g \rho_w A_{wp},$
%we have
%\begin{equation}
%\label{Hamiltonian}
%\begin{array}{lcl}K =\frac{1}{2}\mathbf{m}^T\ T^{-1} \mathbf{m} + \frac{1}{2}\mathbf{p}^T m_v^{-1}\mathbf{p},\\
%U= \frac{1}{2}\mbox{\boldmath $\mu$}^T\tilde{\mathcal{G}}\mbox{\boldmath $\mu$}+\frac{1}{2}\mathbf{q}_1^T\mathbf{q}_1+\frac{1}{2}\mathbf{q}_2^T\mathbf{q}_2 + \frac{1}{2}\mathbf{q}_3^T\mathbf{q}_3+ \frac{1}{2}\mathbf{x}^T\mathcal{A}\mathbf{x},\\
%H=K+U.
%\end{array}
%\end{equation}
%%with
%%$$\mathcal{A}  := \mathrm{diag}(0,0,c), \quad \mathcal{G}  := m_v g\, \mathrm{diag}(\overline{GM}_L,\overline{GM}_T,0).$$
%%and $c := g \rho_w A_{wp}.$
%Notice that the following identities hold
%\begin{equation}
%\label{gtsgrs}
%\mathbf{g}_t^s=\mathcal{A}\, \mathbf{x},\quad Q^T\mathbf{g}_r^s=\mbox{\boldmath $\mu$}\times \mathbf{q}_3.
%\end{equation}
%We will in the next proposition replace the matrix equation $\dot{Q}=Q\hat{\boldsymbol{\omega}}$ in \eqref{eq:vessel} by three vector equations, one for each column $\mathbf{q}_i$, $i=1,2,3$ of $Q^T$.
%
%\begin{Proposition}
%\label{portHamSys}
%The system \eqref{eq:vessel} can be written in the form
%\begin{equation}
%\label{eq:xiDiff}
%\dot{\mbox{\boldmath $\xi$}} = S(\mbox{\boldmath $\xi$})\nabla H(\mbox{\boldmath $\xi$}) -\tilde{I}\left(D(\mbox{\boldmath $\xi$})\mbox{\boldmath $\nu$} - \tilde{\mbox{\boldmath $\tau$}}\right),
%\end{equation}
%with
%\begin{equation}
%\label{eq:skewMat}
%S(\mbox{\boldmath $\xi$}) := \begin{bmatrix} 
%0_{3 \times 3} & \widehat{\mathbf{p}} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  0_{3 \times 3} &-Q^T \\ 
% \widehat{\mathbf{p}} &\widehat{\mathbf{m}} & 0_{3 \times 3} &0_{3 \times 3} & -\widehat{\mbox{\boldmath $\mu$}} & 0_{3 \times 3}  & 0_{3 \times 3}\\ 
%%0_{3 \times 3} & -m_v\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  0_{3 \times 3} &-Q^T \\ 
% 0_{3 \times 3} &  0_{3 \times 3} & -\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3} & 0_{3 \times 3} &0_{3 \times 3} & 0_{3 \times 3}\\
% 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} &  -\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3}  &   0_{3 \times 3} & 0_{3 \times 3}\\
% 0_{3 \times 3} & -\widehat{\mbox{\boldmath $\mu$}} &  0_{3 \times 3} &   0_{3 \times 3} &   -\widehat{T^{-1}\mathbf{m}} &   -\widehat{T^{-1}\mathbf{m}}\,\mathcal{G}  & 0_{3 \times 3}\\
% 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & 0_{3 \times 3} & -\mathcal{G}\,\widehat{T^{-1}\mathbf{m}} & 0_{3 \times 3} & 0_{3 \times 3}\\
%Q & 0_{3 \times 3} &  0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} &   0_{3 \times 3} & 0_{3 \times 3}
%\end{bmatrix}, \ \ 
%\tilde{I} := \begin{bmatrix} 
%I{\ensuremath{_{6\times6}}} \\
%0{\ensuremath{_{15\times6}}}
%\end{bmatrix},
%\end{equation}
%$$D(\mbox{\boldmath $\xi$}):=D+\left[\begin{array}{cc} Q  & \Z3x3 \\
%\Z3x3 & \Pi_e^{-1}Q \end{array} \right]^TK_d \left[\begin{array}{cc} Q & \Z3x3 \\
%\Z3x3 & \Pi_e^{-1}Q\end{array} \right],$$
%and
%$$\tilde{\mbox{\boldmath $\tau$}}=\mbox{\boldmath $\tau$}-\left[\begin{array}{cc} Q & \Z3x3 \\
%\Z3x3 & \Pi_e^{-1}Q \end{array} \right]^TK_d \left[\begin{array}{cc} Q & \Z3x3 \\
%\Z3x3 & \Pi_e^{-1}Q \end{array} \right] \mbox{\boldmath $\nu$} $$
%
%$$\tilde{\mbox{\boldmath $\tau$}}=\left[\begin{array}{cc} Q & \Z3x3 \\
%\Z3x3 & \Pi_e^{-1}Q \end{array} \right]^T \left[\begin{array}{c}
%K_p^{r}\tilde{\mbox{\boldmath $\theta$}}+K_i^{r} \mbox{\boldmath $\varphi$}_{\boldsymbol{\theta}}\\
%K_p^{t}\tilde{\mathbf{x}}+K_i^{t} \mbox{\boldmath $\varphi$}_{\mathbf{x}}
%\end{array}\right]$$
%
%%\begin{align*}
%%\dot{\mbox{\boldmath $\varphi$}}_{\boldsymbol{\theta}}&=\tilde{\mbox{\boldmath $\theta$}}, \nonumber\\
%%\dot{\mbox{\boldmath $\varphi$}}_{\mathbf{x}} &=\tilde{\mathbf{x}}, \nonumber
%%\end{align*}
%with 
%
%\begin{align*}
%%\mbox{\boldmath $\tau$}_r  &= -\left(\Pi_e^{-1}Q)^T(K_p^{r}\tilde{\mbox{\boldmath $\theta$}}
%%+ K_d^{r}\dot{\tilde{\mbox{\boldmath $\theta$}}} + K_i^{r} \mbox{\boldmath $\varphi$}_{\boldsymbol{\theta}}\right), \\
%%\int_{t_0}^t \! \tilde{\mbox{\boldmath $\theta$}}(\sigma) \,d\sigma), 
%%\boldsymbol{\tau}_t &= -Q^T \left(K_p^{t}\tilde{\mathbf{x}}
%%+ K_d^{t}\dot{\tilde{\mathbf{x}}} + K_i^{t} \mbox{\boldmath $\varphi$}_{\mathbf{x}}\right),\\
%\tilde{\mbox{\boldmath $\theta$}} &= \mbox{\boldmath $\theta$}- \mbox{\boldmath $\theta$}_{ref}, %= J(\mbox{\boldmath $\eta$})
%%\mbox{\boldmath $\nu$} \hspace{3mm} \implies 
%\hspace{6mm}
%\dot{\tilde{\mbox{\boldmath $\theta$}}} = \dot{\mbox{\boldmath $\theta$}} = \Pi_e^{-1}Q\, \mbox{\boldmath $\omega$} ,
%\hspace{6mm}
%\tilde{\mathbf{x}} = \mathbf{x}-\mathbf{x}_{ref},
%\hspace{6mm}
%\dot{\mbox{\boldmath $\varphi$}}_{\boldsymbol{\theta}} =\tilde{\mbox{\boldmath $\theta$}}
%\hspace{6mm}
%\dot{\mbox{\boldmath $\varphi$}}_{\mathbf{x}} =\tilde{\mathbf{x}}.
%\end{align*}
%
%\end{Proposition}
%\begin{proof}
%The proof follows by a direct calculation of the gradient of $H$. 
%\end{proof}
%
%
%\vspace{1em}




